Can MLLMs Perform Text-to-Image In-Context Learning?

The evolution from Large Language Models (LLMs) to Multimodal Large Language Models (MLLMs) has spurred research into extending In-Context Learning (ICL) to its multimodal counterpart. Existing such studies have primarily concentrated on image-to-text ICL. However, the Text-to-Image ICL (T2I-ICL), with its unique characteristics and potential applications, remains underexplored. To address this gap, we formally define the task of T2I-ICL and present CoBSAT, the first T2I-ICL benchmark dataset, encompassing ten tasks. Utilizing our dataset to benchmark six state-of-the-art MLLMs, we uncover considerable difficulties MLLMs encounter in solving T2I-ICL. We identify the primary challenges as the inherent complexity of multimodality and image generation, and show that strategies such as fine-tuning and Chain-of-Thought prompting help to mitigate these difficulties, leading to notable improvements in performance. Our code and dataset are available at https://github.com/UW-Madison-Lee-Lab/CoBSAT.

==> abstract_old.tex <==
\begin{abstract}
The evolution from Large Language Models (LLMs) to Multimodal Large Language Models (MLLMs) has spurred research into extending In-Context Learning (ICL) to its multimodal counterpart.
Existing such studies have primarily concentrated on image-to-text ICL.
However, the Text-to-Image ICL (T2I-ICL), with its unique characteristics and potential applications, remains underexplored. 
To address this gap, we formally define the task of T2I-ICL and present \textbf{\ours{}}, the first T2I-ICL benchmark dataset, encompassing ten tasks.
Utilizing our dataset to benchmark six state-of-the-art MLLMs, we uncover considerable difficulties MLLMs encounter in solving T2I-ICL. 
We identify the primary challenges as the inherent complexity of multimodality and image generation. 
To overcome these challenges, we explore strategies like fine-tuning and Chain-of-Thought prompting, demonstrating notable improvements.
Our code and dataset are available at \url{https://github.com/UW-Madison-Lee-Lab/CoBSAT}.
\end{abstract}


==> main_body_old.tex <==
\section{Introduction}

\input{tex/figures/fig_intro}
\input{tex/figures/fig_overview}

In the past two years, Large Language Models (LLMs)~\citep{devlin2018bert,radford2019gpt2,brown2020gpt3,openai2023gpt4,touvron2023llama} have gained significant attention for their wide-ranging applications. 
They excel in tasks such as interpreting language-format questions, surpassing human performance in exams like the GRE and SAT~\citep{openai2023gpt4}, refining writing~\citep{openai2023gpt4}, and assisting in research~\citep{huang2023researchagent}. 

The emergence of Multimodal Large Language Models (MLLMs)~\citep{ge2023seed2,koh2023gill,sun2023emu,openai2023gpt4,liu2023llava1.5,bai2023qwen,geminiteam2023gemini,li2023blip2} marks a significant advancement, handling not only text but also images, videos, and audio. 
This multimodal capability enables MLLMs to undertake complex tasks, integrating visual, auditory, and textual cues. 
The versatility of MLLMs makes them powerful tools in AI, offering context-rich interpretations across various domains.

In-Context Learning (ICL) (see Figure~\ref{fig:intro}(a)) is a prevalent technique that enables predictions based on context through a sequence of input-output pairs, termed demonstrations, without requiring any model parameter updates. 
This capability was initially identified and applied by \citet{brown2020gpt3} and has since become a widely used standard prompt engineering method to enhance LLM inference performance for various downstream tasks. 
This method has been applied in computer vision to produce output images contextually aligned with provided image-image pair examples, termed Visual ICL (V-ICL) (see Figure~\ref{fig:intro}(b))~\citep{bar2022visual,wang2023painter}.
In another development, \citet{tsimpoukelli2021multimodal} introduced Multimodal ICL (M-ICL) for the first time for image-to-text generation tasks, including applications such as visual question answering and image captioning. 
Unlike ICL, which is exclusively text-focused, and V-ICL, which is solely image-oriented, M-ICL uses demonstrations that incorporate samples from two modalities.

The majority of existing M-ICL work~\citep{tsimpoukelli2021multimodal,alayrac2022flamingo,monajatipoor2023metavl,chen2023understanding,zhao2023mmicl} has mainly centered on the performance of image-to-text tasks, the goal of which is transforming high-dimensional, image-based input into low-dimensional, text-based output. 
However, when the roles are reversed, and low-dimensional inputs (text) are used to generate high-dimensional outputs (images or videos), models can exhibit significantly different performance characteristics. 
To distinguish between these two tasks, we refer to M-ICL for image-to-text generation as \emph{Image-to-Text ICL} (I2T-ICL) (see Figure~\ref{fig:intro}(c)), and M-ICL for text-to-image generation as \emph{Text-to-Image ICL} (T2I-ICL) (see Figure~\ref{fig:intro}(d)), with the latter being the focus of our work. 
It is important to note that potential applications of T2I-ICL are completely different from I2T-ICL, which include areas like product design and personalized content creation.


A concurrent work by \citet{sun2023emu2} explored T2I-ICL capabilities, utilizing the DreamBooth dataset~\citep{ruiz2023dreambooth}, previously known for its application in fine-tuning diffusion models~\citep{sohl2015diffusion}. 
However, DreamBooth was not originally designed for T2I-ICL, but for specific task-based model fine-tuning. 
This inherent design gap poses significant challenges for evaluating T2I-ICL.
A key limitation is the dataset's narrow focus, which primarily centers on background alterations in images. 
While there are a few examples for other tasks such as style transfer, their complexity often exceeds current MLLM's T2I-ICL capabilities and is more suited to fine-tuning tasks. 
For instance, their examples of style transfers involving styles attributed to artists like Vincent van Gogh or Michelangelo can be too complicated for T2I-ICL, as they can also be difficult for humans to discern.

\subsection{Our Contributions}

\paragraph{Identifying an Important Problem: T2I-ICL.} 
Our work first identifies the important yet underexplored ICL setting with a particular focus on text-to-image generation, termed T2I-ICL.
T2I-ICL is distinct from most existing ICL settings, and opens doors to a variety of useful applications like product design and personalized content generation.

\paragraph{Introducing \ours{} Benchmark.} To systematically assess the capability of MLLMs in learning to map low-dimensional text inputs to high-dimensional image outputs from in-context demonstrations, we introduce a comprehensive benchmark featuring tasks across five different themes — \textbf{Co}lor, \textbf{B}ackground, \textbf{S}tyle, \textbf{A}ction, and \textbf{T}exture, which is named as \textbf{\ours{}}.
Each theme comprises 100 images, allowing us to examine whether MLLMs can easily adapt the same or different color, background, style, action, and texture for the same or different objects.
For example, as illustrated in Figure~\ref{fig:overview_data}, we provide two in-context demonstrations in each prompt.
Each demonstration consists of a textual input (\eg, ``white'') and an image output (\eg, an image of a white car). 
We expect the model to generate an image based on the text, and the correct image can only be generated if the model understands both the textual query (\eg, ``red'') and the relationship between the text input and the image output (\eg, a car of the specified color) as presented in the in-context demonstrations.
Furthermore, our dataset includes two variants, differentiated by inference focus. 
For each variant, we provide a total of 1,000 prompts for each theme, resulting in a total of 10,000 prompts for a setting with a fixed number of in-context demonstrations.

\paragraph{Benchmarking MLLMs in T2I-ICL.}
We utilize our dataset to evaluate the T2I-ICL capabilities of six leading MLLMs.
These models include Emu~\citep{sun2023emu}, GILL~\citep{koh2023gill}, SEED-LLaMA~\citep{ge2023seed2}, LLaVA~\citep{liu2023llava1.5}, Qwen-VL~\citep{bai2023qwen}, and GPT-4V~\citep{openai2023gpt4}. 
Among them, SEED-LLaMA, Qwen-VL, and GPT-4V emerge as the top performers. 
However, even these models demonstrate only about 60\% accuracy or lower in most scenarios. 
Moreover, the accuracy does not improve with the addition of more in-context demonstrations, highlighting the challenges MLLMs face in effectively conducting T2I-ICL. 

\paragraph{Understanding Challenges in T2I-ICL.}
We then investigate the key factors contributing to the underperformance of MLLMs in T2I-ICL. 
Our findings point to two principal challenges: (i) the intrinsic complexity involved in processing multimodal data, and (ii) the inherent difficulties associated with the task of image generation.

\paragraph{Enhancing MLLMs' T2I-ICL Capabilities.}
To augment MLLMs' T2I-ICL capabilities, we delve into various potential techniques. 
Our study demonstrates that fine-tuning significantly boosts T2I-ICL performance.
While prompt engineering methods such as Chain-of-Thought (CoT)~\citep{wei2022chain} and the inclusion of clear task descriptions show promising results on specific MLLMs, a more detailed examination is needed for them to achieve consistent improvements in T2I-ICL.

\section{Related Works}
\paragraph{Textual ICL.} 
Ever since \citet{brown2020gpt3} demonstrated that language models are in-context learners (see Figure~\ref{fig:intro}(a)), there has been substantial interest in comprehending this capability, both empirically~\citep{liu2022what,min2022rethinking,chen2022meta,mishra2022reframing,lampinen2022language,garg2022what,hendel2023context} and theoretically~\citep{xie2022an,wies2023learnability,akyurek2023what,von2023transformers,bai2023transformers,ahn2023transformers,zhang2023trained}. 
Textual ICL (T-ICL) enables the adaptation of LLMs to downstream tasks simply by providing a few illustrative examples, bypassing any need for updating model parameters. 
The existing works indicate that LLMs possess the capability to comprehend context and perform reasoning through T-ICL~\citep{brown2020gpt3}.

\paragraph{Visual ICL.} 
The concept of V-ICL is then employed in computer vision, starting with the introduction of visual prompts (see Figure~\ref{fig:intro}(b)). 
The pioneering works by \citet{bar2022visual,wang2023painter} propose to automatically generate output images that are contextually aligned with provided examples.
Specifically, \citet{bar2022visual} developed a method that combines three images - an example input, its corresponding output, and a query - into a single composite image.
In this layout, the example input is placed in the upper left, the example output in the upper right, the query image in the bottom left, and the bottom right patch is left blank for output construction via an image inpainting model. 
\citet{bar2022visual} demonstrated the effectiveness of V-ICL in tasks like edge detection, colorization, inpainting, segmentation, and style transfer. 
\citet{wang2023painter} introduced a similar approach and trained a generalist model named ``Painter,'' which exclusively uses visual prompts without any textual data for V-ICL.
Experiments on standard computer vision benchmarks revealed competitive performance against task-specific models. 
\citet{nguyen2023visual} further applied visual prompts to image editing by inverting visual prompts into text-based editing directions, leveraging the pre-trained capabilities of diffusion models.

A subsequent empirical study by \citet{zhang2023makes} highlighted that the success of V-ICL significantly depends on the choice of in-context demonstrations.
The aspect of demonstration selection was further explored by \citet{sun2023exploring}, who also examined the impact of prompt fusion on performance. 
Their findings indicate a high sensitivity of performance to the arrangement of sub-images in in-context learning.
Moreover, innovative approaches to structuring V-ICL, such as the concept of ``visual sentences,'' have been introduced in recent studies, notably by \citet{bai2023sequential}.
Unlike V-ICL which only handles images, M-ICL integrates demonstrations encompassing both text and images.

\paragraph{MLLMs.} 
In light of the significant success of LLMs, there has been an increase in the release of MLLMs. 
These models are designed to address more challenging multimodal tasks, thereby enabling the perception of images~\citep{li2022blip,alayrac2022flamingo,hao2022metallm,laurenccon2023obelisc,huang2023kosmos,peng2023kosmos2,li2023blip2,ge2023seed2,koh2023gill,zhu2023minigpt4,sun2023emu,zheng2023minigpt5,openai2023gpt4,liu2023llava,liu2023llava1.5,bai2023qwen,sun2023emu2,geminiteam2023gemini,driess2023palm}, videos~\citep{li2022blip,alayrac2022flamingo,li2023blip2,sun2023emu,geminiteam2023gemini}, and audio~\citep{hao2022metallm,borsos2023audiolm,huang2023audiogpt,chen2023lauragpt,zhang2023speechgpt,geminiteam2023gemini}.
Existing models capable of handling images can be categorized as follows: 
(i) those that use language as a general interface and directly employ LLMs without altering the model architectures~\citep{dinh2022lift,cai2023leveraging,aghajanyan2022cm3,yu2023cm3leon,huang2023kosmos,mirchandani2023large,cai2023leveraging}; 
(ii) those that add one or more modules before feeding the input sequence into the LLM to perceive multimodal inputs~\citep{tsimpoukelli2021multimodal,alayrac2022flamingo,awadalla2023openflamingo,laurenccon2023obelisc,li2023blip2,hao2022metallm,liu2023llava,liu2023llava1.5,zhu2023minigpt4}; 
(iii) those that add one or more modules after the LLM processing for generating multimodal outputs~\citep{pan2023kosmosg};
(iv) those that add modules to both inputs and outputs of the LLMs to process the multimodal input and generate multimodal outputs~\citep{dong2023dreamllm,sun2023emu,koh2023gill,ge2023seed2,zheng2023minigpt5}.

In this paper, our main focus is T2I-ICL. 
We aim to investigate whether MLLMs can learn to transform low-dimensional textual input into high-dimensional visual output based on demonstrations, and to accurately generate images from new textual queries.
Consequently, we focus on models capable of processing both text and multiple images. We consider two types of MLLMs: (i) proficient in generating both text and images, including Emu~\citep{sun2023emu}, GILL~\citep{koh2023gill}, and SEED-LLaMA~\citep{ge2023seed2}, and (ii)  those limited to text generation, including GPT-4V~\citep{openai2023gpt4}, LLaVA~\citep{liu2023llava}, and Qwen-VL~\citep{bai2023qwen}.
For text-only MLLMs, we evaluate their capacity to infer visual outputs by prompting them to describe the anticipated image. 
Conversely, for MLLMs capable of image generation, we not only elicit image outputs but also ask for descriptive text, ensuring an apple-to-apple comparison with text-only models.


\paragraph{Image-to-Text ICL in MLLMs.}
Most existing work on M-ICL focuses on the image-to-text generation, \ie, I2T-ICL, which involves mapping from high-dimensional input (\ie, images) to low-dimensional output (\ie, text).
In particular, \citet{tsimpoukelli2021multimodal} were the first to extend ICL from the text domain to the multimodal domain, focusing on image-to-text generation such as visual question-answering (see Figure~\ref{fig:intro}(c)). 
\citet{alayrac2022flamingo} introduced Flamingo, an MLLM that achieves state-of-the-art performance in a variety of image and video understanding tasks using I2T-ICL with 32 demonstrations, implying the efficacy of I2T-ICL in performance enhancement in their model. 
In contrast, \citet{monajatipoor2023metavl} explores whether the in-context capabilities of LLMs can be seamlessly extended to I2T-ICL by incorporating a visual encoder.
\citet{chen2023understanding} conducted a systematic study on the importance of visual and textual information in I2T-ICL.
Concurrently, efforts have been made to develop datasets specifically designed for evaluating I2T-ICL capability of MLLMs~\citep{zhao2023mmicl}.
In contrast, there have been only a few attempts~\citep{sun2023emu2} to evaluate the T2I-ICL capability of MLLMs, a domain that remains relatively unexplored compared to its image-to-text counterpart.

\paragraph{Zero-Shot Image Generation in MLLMs.}
A relatively small number of MLLMs are capable of image generation~\citep{yu2023cm3leon,dong2023dreamllm,zheng2023minigpt5,sun2023emu,ge2023seed2,koh2023gill,pan2023kosmosg,sun2023emu2,geminiteam2023gemini}. 
Zero-shot text-to-image generation typically generates images directly from textual descriptions without relying on any examples. 
This does not require the model to integrate a combination of textual and visual inputs.
Another common task for MLLMs in image generation is context modifications. 
In this more complex scenario, the model receives visual inputs (\eg, an image of a dog) along with associated textual instructions (\eg, ``swimming underwater'').
This task requires a nuanced understanding and manipulation of the image, guided by the textual instructions, thereby blending image comprehension with contextual transformation based on text.
Unlike zero-shot image generation, our focus is on studying whether MLLMs can learn the implicit relationship between the input and output from multiple in-context demonstrations.

\paragraph{Text-to-Image ICL in MLLMs.}
There are limited attempts to evaluate MLLMs based on their T2I-ICL capabilities. 
A notable exception is concurrent research by \citet{sun2023emu2}. 
They evaluated the performance of their model on T2I-ICL with DreamBooth dataset~\citep{ruiz2023dreambooth}.
However, it is important to note that the DreamBooth dataset, primarily developed for fine-tuning models to modify image contexts, was not specifically designed for T2I-ICL applications. 
This leads to certain constraints, such as its concentrated emphasis on altering backgrounds only and a level of complexity that may not align well with T2I-ICL.
In contrast, our dataset spans five themes and provides well-designed prompts to assess whether models can understand both visual and textual information, learn mappings from demonstrations, and make inferences.

\paragraph{Image Evaluation Metrics.}
A variety of metrics exist for assessing the quality of generated images. 
Classical ones like Peak Signal-to-Noise Ratio (PSNR)~\citep{wang2004image} evaluate the quality of reconstructed images or videos by measuring pixel-level errors compared to the target images. 
Fr\'echet Inception Distance (FID)~\citep{parmar2022aliased} gauges the quality of images produced by generative models, such as Generative Adversarial Networks, by calculating the similarity between the distributions of generated and real images. 
However, these metrics are not entirely suitable for our purpose, where no single definitive ground-truth target image exists but rather a textual label (\eg, ``red car'' in the first example of Figure~\ref{fig:overview_data}).

In the realm of text-to-image generation, the CLIP similarity~\citep{radford2021clip} metric has gained popularity~\citep{ruiz2023dreambooth}. 
It measures the cosine similarity between the CLIP embeddings of the textual ground truth and the visual output. 
Meanwhile, there is a growing trend of utilizing MLLMs for evaluation~\citep{zhang2023gpt,hu2023tifa}, showing promising results in text-to-image tasks. 
Our study embraces this approach, utilizing LLaVA~\citep{liu2023llava1.5} to assess the accuracy of generated images. 
This accuracy metric is more interpretable than the CLIP similarity. 
To be more specific, we utilize LLaVA to identify the object (\eg, ``car'') and attribute (\eg, ``red'') in the image generated by MLLMs and then compare these identifications with the actual label (\eg, ``red car'' for the first example in Figure~\ref{fig:overview_data}). 
We have confirmed LLaVA's effectiveness in accurately recognizing the object and attribute in these images, as evidenced by its 100\% accuracy rate in correctly labeling the objects and attributes of images within our dataset.
Additionally, we examine the correlation between the accuracy calculated by LLaVA and CLIP similarity to further validate the efficacy of using LLaVA as our evaluation tool in Sec.~\ref{app:clip}.

\section{Dataset: \ours{}}\label{sec:dataset}
We start by describing the definition of in-context learning. 
Consider a task with data $(x, y)$, where input $x \in \gX$, output $y \sim f_{\theta}(x)$, where distribution $f_{\theta}$ is parameterized by latent variable $\theta \in \Theta$.
We denote the model by $M$.
For in-context demonstrations, we are given $N$ input-output pairs $\set{(x_n, y_n)}_{n=1}^N$ and one test query $x_{N+1}$.
In-context learning make the prediction by incorporating these demonstrations $\set{(x_n, y_n)}_{n=1}^N$ and the test query $x_{N+1}$ in the prompt. 
The prediction made by model $M$ is formulated as $\hy_{N+1} = M(x_1, y_1, x_2, y_2, \ldots, x_N, y_N, x_{N+1})$.

In this work, we mainly focus on scenarios where the input $x$ is textual data and output $y$ corresponds to an image. 
We use notation \img{description} to denote an image corresponding to the text description. 
For instance, \img{red car} refers to an image depicting a red car.

\input{tex/tables/tab_tasks}

\paragraph{Dataset Structure.} 
We begin by outlining the structure of our dataset, which evaluates whether models are capable of learning the mapping from low-dimensional textual input to high-dimensional visual output, based on the given in-context demonstrations.
For instance, task Color-I in our experiment involves generating an image of an object of a particular color, where the object to be drawn is not explicitly stated in the text data $x_{N+1}$. 
The information of the object is instead implicitly contained in $\theta$ (and hence in $y_i$'s since $y_i \sim f_{\theta}(x_i)$ for all $i = 1,\ldots,N$), which can be learned from the in-context demonstrations. 
An example prompt with two demonstrations when $\theta = \text{``car''}$ is
\begin{equation}
    \text{``}\overbrace{\underbrace{\text{red:}}_{x_1}~\underbrace{\text{\img{red car}}}_{y_1}}^{\text{example 1}}~\overbrace{\underbrace{\text{blue:}}_{x_2}~\underbrace{\text{\img{blue car}}}_{y_2}}^{\text{example 2}}~\overbrace{\underbrace{\text{pink: }}_{x_3}}^{\text{query}}.\text{''}
\end{equation}
Ideally, MLLMs can learn the object $\theta$ from the context, and then generate an image of a pink car.

\ours{} comprises ten tasks, divided into two categories: (i) \emph{object-inference tasks}, which give the attributes (\eg, color, texture) in the text input and require identifying objects (\eg, car, cup) from images, and (ii) \emph{attribute-inference tasks}, which provide the object to be drawn in the text input but require identifying the common attribute from the images.
Each task has predefined lists for text inputs and latent variables, denoted as $\gX$ and $\Theta$, each containing ten distinct items. 
For instance, in the Color-I task, the predefined list for the latent variable (\ie, the object) is $\Theta = \{$leaf, hat, cup, chair, car, box, book, ball, bag, apple$\}$, and the predefined list for the text input (\ie, the attribute) is $\gX = \{$yellow, white, red, purple, pink, orange, green, brown, blue, black$\}$. 
The predefined lists for all tasks are provided in Table~\ref{tab:datasets}.
In our experiment, for each specified number of shots (\ie, 2, 4, 6, 8 in our experiments), we create 1,000 prompts per task.
This is accomplished by randomly selecting a latent variable $\theta$ from the predefined list $\Theta$ and a sequence of textual inputs $(x_n)_{n=1}^{N+1}$ from $\gX^{N+1}$. 
Then, we pair each textual input $x_n$ with the corresponding image $y_n \sim f_{\theta}(x_n)$ to instruct in-context demonstrations.
The images are collected from the web and DaLL-E 3~\citep{betker2023dalle3}.

\paragraph{Data Collection.}
For each task outlined in Table~\ref{tab:datasets}, we gather one image for every possible pairing of the textual input $x \in \gX$ and latent variable $\theta \in \Theta$, resulting in $\left|\gX\right| \times \left|\Theta\right| = 10\times 10=100$ images for each task. 
For instance, for task Color-I, we collect an image of a red car to correspond to the case where $x=$``red'' and $\theta=$``car,'' and likewise for other images.
It is noteworthy that the tasks with the same theme, such as Color-I (object-inference task) and Color-II (attribute-inference task), share the same images. 
In addition, all object lists and attribute lists presented in Table~\ref{tab:datasets}, along with the images, are carefully selected so that LLaVA can correctly identify the specified objects and the corresponding attributes (\ie, color, background, texture, action, and style) of the images.
This ensures an appropriate level of difficulty for T2I-ICL tasks and allows LLaVA to perform reliable evaluations on generated images.
In total, we collect 500 images from the web and DALL-E~3~\citep{betker2023dalle3}.
We then construct in-context prompts for 2, 4, 6, and 8 shots as previously described, with each shot resulting in 10,000 prompts in total. 

\section{Methodology and Experiment Setup}\label{sec:setup}
In this section, we introduce the MLLMs under evaluation and describe the evaluation pipeline, which is summarized in Figure~\ref{fig:framework_flow}.
Recognizing that many MLLMs lack the capability to generate images, we include the text-only generating MLLMs by prompting them to generate image descriptions instead of images. 

\input{tex/figures/fig_framework}

\subsection{MLLMs} 
We apply T2I-ICL on (i) three MLLMs with image generation capabilities: Emu~\citep{sun2023emu}, %
SEED-LLaMA~\citep{ge2023seed1,ge2023seed2}, and GILL~\citep{koh2023gill}; (ii) three state-of-the-art MLLMs that can only generate text: Qwen-VL~\citep{bai2023qwen}, LLaVA~\citep{liu2023llava1.5} and GPT-4V~\citep{openai2023gpt4}.

Emu, SEED-LLaMA, and GILL enhance their multimodal functionalities by integrating both vision encoders and decoders with an LLM.
Specifically, Emu~\citep{sun2023emu} utilizes EVA-CLIP~\citep{fang2023eva} as the visual encoder, LLaMA-13B~\citep{touvron2023llama} as the LLM, and Stable Diffusion v1.5~\citep{rombach2022latentdiffusion} as the visual decoder.
SEED-LLaMA~\citep{ge2023seed2}, particularly SEED-LLaMA-14B used in our experiments, employs the SEED tokenizer~\citep{ge2023seed1}, integrating a ViT encoder~\citep{dosovitskiy2021an} from BLIP-2~\citep{li2023blip2}, a Causal Q-Former from VQ book~\citep{van2017neural}, and a multi-layer perceptron for processing image inputs.
It uses LLaMA2-chat-13B~\citep{touvron2023llama} as the LLM and a UNet decoder~\citep{ronneberger2015unet} from unCLIP~\citep{ramesh2022unclip}, along with the Stable Diffusion model for image generation. 
GILL~\citep{koh2023gill} introduces GILLMapper~\citep{koh2023gill}, featuring a Transformer encoder, and employs Stable Diffusion v1.5 to generate realistic images. 
Its LLM backbone is OPT-6.7B~\citep{zhang2022opt}.
In contrast, Qwen-VL and LLaVA extend LLMs with a single visual encoder to process visual inputs. 
Qwen-VL~\citep{bai2023qwen} integrates a Vision Transformer (ViT)~\citep{dosovitskiy2021an} from OpenCLIP's ViT-bigG~\citep{ilharco_gabriel_2021_5143773} and a cross-attention module, converting images into sequences for the Qwen-7B LLM~\citep{qwen-language}. 
LLaVA~\citep{liu2023llava,liu2023llava1.5}, based on Vicuna-v1.5-13B LLM~\citep{chiang2023vicuna}, includes CLIP-ViT-L-336px~\citep{radford2021clip} and an MLP projection for encoding visual features. 
Lastly, GPT-4V~\citep{openai2023gpt4}, known for its superior performance, remains closed-sourced with undisclosed architectural details.

In our study, we assess the performance of models in T2I-ICL, specifically Emu, SEED-LLaMA, and GILL, which can generate images.
In addition to image generation scenarios, we instruct the models, particularly text-only generation models (\ie, Qwen-VL, LLaVA, and GPT-4V), to generate textual descriptions for image predictions. 
This assesses if they can learn the mapping from low-dimensional textual input to high-dimensional visual output based on the demonstrations.
Detailed information about the prompts used for each model, as well as an extensive review of these MLLMs, are provided in Sec.~\ref{app:prompt} and Sec.~\ref{app:mllm}, respectively.

\begin{figure*}[!htb]
    \centering
    \begin{subfigure}[b]{\textwidth}
        \includegraphics[width=\textwidth]{figures/object_inference_m_0_image.pdf}
        \caption{Accuracy of generated images on object-inference tasks in \ours{}.}
        \label{fig:object_inference_m_0_image}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}
        \includegraphics[width=\textwidth]{figures/detail_inference_m_0_image.pdf}
        \caption{Accuracy of generated images on attribute-inference tasks in \ours{}.}
        \label{fig:detail_inference_m_0_image}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}
        \includegraphics[width=\textwidth]{figures/object_inference_m_0_text.pdf}
        \caption{Accuracy of generated image descriptions on object-inference tasks in \ours{}.}
        \label{fig:object_inference_m_0_text}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}
        \includegraphics[width=\textwidth]{figures/detail_inference_m_0_text.pdf}
        \caption{Accuracy of generated image descriptions on attribute-inference tasks in \ours{}.}
        \label{fig:detail_inference_m_0_text}
    \end{subfigure}
    \caption{
        \textbf{Performance of MLLMs on \ours{} benchmark.}
        We evaluate the T2I-ICL performance of various MLLMs with 2,4,6,8 in-context demonstrations.
        In particular, (a) and (b) are evaluated on generated images of the considered MLLMs with image generation capabilities, on object-inference and attribute-inference tasks, respectively; (c) and (d) visualize the accuracy of generated image descriptions of all considered MLLMs on these tasks.
    }
    \label{fig:overall_vis}
\end{figure*}



\subsection{Evaluation Pipeline}
In this section, we present our evaluation pipeline, which is summarized in Figure~\ref{fig:framework_flow}. 
The evaluation encompasses two scenarios: (i) assessing the generated images, and
(ii) assessing the generated image descriptions.


\paragraph{Assessing Generated Images.}
We employ LLaVA to evaluate the generated images in terms of whether they generated the right object (\eg, ``car'' in the first example in Figure~\ref{fig:overview_data}) and attribute (\eg, ``red'' in the first example in Figure~\ref{fig:overview_data}).
To facilitate this evaluation, we design specific prompts for LLaVA. 
Here are the prompts designed for tasks Color-I and II:
\begin{itemize}[leftmargin=*]
    \item Object Identification: \textit{``\img{generated image} What is the main object in this image? Answer from the following options: (1)leaf (2)hat (3)cup (4)chair (5)car (6)box (7)book (8)ball (9)bag (10)apple. Answer the number only and do not include any other texts (e.g., 1).'' }
    \item Attribute Identification: \textit{``\img{generated image} What is the color (of the main object) in this image? Answer from the following options:  (1)yellow (2)white (3)red (4)purple (5)pink (6)orange (7)green (8)brown (9)blue (10)black. Answer the number only and do not include any other texts (e.g., 1).''}
\end{itemize}
For other tasks involving different themes, the options and the attribute category (\eg, replace ``color'' in the attribute inference prompt with ``style'' for tasks Style-I and II) are updated correspondingly. 
We choose LLaVA as our evaluation model since it is one of the most effective freely available MLLMs in visual question answering, notably surpassing Qwen-VL~\citep{liu2023llava1.5}.
Note that we have confirmed that LLaVA can accurately identify the correct object and attribute for the images in our dataset when using the prompts described above. 
This ensures the reliability of our evaluation results.
We further compare our metric with the evaluation analysis performed by CLIP in Sec.~\ref{app:clip}.

\paragraph{Assessing Generated Image Descriptions.} 
We also use LLaVA to evaluate the generated image descriptions. 
However, in this case, we modify the prompts used for assessing generated images by replacing ``\img{generated image}'' with ``Image caption: \txt{generated description}.''

\section{Benchmarking MLLMs in T2I-ICL}\label{sec:basic_exp}
In this section, we present and analyze our experiment results on the evaluation of the considered MLLMs' performance on T2I-ICL. 
The overall performance of the considered MLLMs is visualized in Figure~\ref{fig:overall_vis}. 
We also explore a more complex variation of our dataset, with detailed descriptions of the experiments and results presented in Sec.~\ref{sec:misleading}.

\subsection{Assessing Generated Images} 
In terms of image generation, we focus on the three MLLMs that have this capability: Emu, GILL, and SEED-LLaMA.
Among these, SEED-LLaMA significantly outperforms the others, as evidenced by Figure~\ref{fig:overall_vis}(a) and (b), achieving a score of 68\% on Color-I tasks.
In contrast, Emu and GILL exhibit low performance, achieving accuracies around or even below 10\%.
For a more tangible understanding, we present specific prompts alongside the images generated using Emu, GILL, and SEED-LLaMA, for task Color-I, as showcased in Figure~\ref{fig:example_prompt_results_main}(a). 
We observe that while both GILL and Emu exhibit low performance, GILL does manage to generate images that either align with the textual query (\eg, ``pink'' in the fourth example of Figure~\ref{fig:example_prompt_results_main}(a)) or adhere to common visual patterns (\eg, ``leaf'' in the sixth example of the same figure).
Conversely, Emu occasionally generates random images, as in the fourth example of Figure~\ref{fig:example_prompt_results_main}(a). 
This phenomenon is further corroborated by numerous additional examples across other tasks, detailed in Sec.~\ref{app:vis}.

\input{tex/figures/fig_prompt_examples_main_body}

\subsection{Assessing Generated Image Descriptions}\label{sec:exp_description}
For image description generation, Figure~\ref{fig:overall_vis}(c) and (d) illustrate the performance of MLLMs in performing T2I-ICL for object-inference and attribute-inference tasks, respectively. 

Our observations indicate that Qwen-VL and GPT-4V significantly outperform other MLLMs on most tasks. 
Specifically, for object-inference tasks, GPT-4V achieves an accuracy of 84.4\%, 84.4\%, 
and 59.2\% on Color-I, Background-I, and Texture-I tasks, respectively, surpassing Qwen-VL, which achieves 56.0\%, 45.9\%, and 45.1\% on the corresponding tasks. 
However, Qwen-VL outperforms GPT-4V on Style-I and Action-I tasks, reaching accuracies of 57.1\% and 67.9\% respectively.
In contrast, for attribute-inference tasks, GPT-4V and Qwen-VL demonstrate similar performance levels.

All other models, except Emu on certain tasks, perform significantly worse than GPT-4V and Qwen-VL, achieving nearly zero performance. 
Emu exhibits outstanding performance on Background-I, Background-II, and Action-II tasks, achieving 70.1\%, 70.7\%, and 75.7\% respectively, but its performance on other tasks is less satisfying. 
As for SEED-LLaMA, its inability to generate text without accompanying images results in poor performance in generating image descriptions. 
This is due to its consistent generation of images paired with the text \textit{``I have generated an image.''}

We offer examples of prompts and their corresponding image descriptions, generated by MLLMs for task Color-I, in Figure~\ref{fig:example_prompt_results_main}(b), and defer more examples for all other tasks, along with the prompts, to Sec.~\ref{app:vis}.
According to the examples, we observe that SEED-LLaMA and GILL often struggle to produce reasonable textual output. 
As previously discussed, SEED-LLaMA predominantly generates images, defaulting to the text \textit{``I have generated an image,''} regardless of varying instructions. 
GILL, on the other hand, tends to produce disjointed sentences like \textit{``image of the backpack in the image.''}
LLaVA's output more frequently describes the images in the prompt rather than accurately predicting the next image.
In contrast, Qwen-VL and GPT-4V demonstrate superior performance, typically generating accurate and reasonable image descriptions. 
Emu also shows commendable performance in this regard.

\subsection{Impact of Number of Demonstrations} 
In this part, we analyze how the number of demonstrations affects the performance of T2I-ICL. 
An interesting observation from Figure~\ref{fig:overall_vis} is the lack of a consistent pattern in how performance is influenced by an increase in the number of demonstrations.
For example, the accuracy in generating image descriptions for models such as Emu, Qwen-VL, and LLaVA initially increases and then decreases with an increasing number of demonstrations generally. 
Conversely, SEED-LLaMA's accuracy first decreases and then increases.

This non-monotonic performance trend with a growing number of demonstrations can potentially be attributed to two factors. 
Firstly, with a higher number of demonstrations, there may be an insufficient number of pertaining samples featuring the corresponding number of image inputs.
For example, LLaVA encounters a context length limitation when presented with eight image inputs, resulting in the model generating only empty strings in 8-shot cases.
Secondly, existing evidence indicates that an increase in demonstrations does not necessarily correlate with enhanced performance~\citep{xie2022an,brown2020gpt3}.
\citet{brown2020gpt3} demonstrate that for some datasets (\eg, LAMBADA, HellaSwag, PhysicalQA, RACE-m, CoQA/SAT analogies for smaller models), GPT-3's zero-shot performance may surpass one-shot performance. 
Similarly, \citet{xie2022an} found that zero-shot scenarios can sometimes outperform few-shot ones, although performance tends to recover with the addition of more examples. 
\citet{xie2022an} posit that an initial decrease in accuracy may be due to the distracting structure of prompts in such settings.
Theoretical insights from \citet{ziqian2023icl} shed light on this phenomenon, suggesting that models initially rely on task retrieval and prior knowledge for predictions with a low number of demonstrations, shifting towards task learning as the number of demonstrations increases.
The presence of a limited number of initial demonstrations might result in the retrieval of an incorrect task, potentially causing a decline in ICL performance.
As more demonstrations are added, performance is anticipated to improve, as the model increasingly depends on task learning, which is improved by a greater number of demonstrations. 
However, in the MLLM scenario, due to the scarcity of prompts with multiple images in the pretrained dataset, we do not anticipate observing this phenomenon.

\subsection{Textual Information v.s. Visual Information}
\begin{figure}[!htb]
    \centering
    \begin{subfigure}[b]{.49\linewidth}
    \centering
        \includegraphics[width=\linewidth]{figures/impact_textual_visual_shot_2_image_0.pdf}
        \caption{Image evaluation}
    \end{subfigure}
        \hfill
    \begin{subfigure}[b]{.49\linewidth}
    \centering
        \includegraphics[width=\linewidth]{figures/impact_textual_visual_shot_2_text_0.pdf}
        \caption{Image description evaluation}
    \end{subfigure}
    \caption{Comparison of alignment with textual information versus visual information when MLLMs perform two-shot T2I-ICL on \ours{} tasks.}
    \label{fig:text_vs_vis}
\end{figure}

In this part, we investigate whether textual or visual information contributes more to the prediction of MLLMs.
We assess this by evaluating how well the output of MLLMs aligns with both types of information. 
For textual alignment, we concentrate on how accurately the models generate images or image descriptions that match the given textual query.
As an example, consider the scenario in Figure~\ref{fig:overview_data}, where the text instructs ``red.''
In this context, we consider the output textually aligned if it features a red object.
We employ a similar approach to measure the visual alignment of the outputs.
Similarly, for visual alignment, we examine whether the generated images or their descriptions accurately incorporate elements from the images presented in the prompts. 
Taking the same example, an output is visually aligned if it correctly represents aspects like ``car,'' which is the common feature in the demonstration images.
Employing these criteria allows us to determine which models are more influenced by textual queries and which lean toward visual cues.

Figure~\ref{fig:text_vs_vis} reveals distinct patterns in how MLLMs respond to these inputs. 
Models like Emu, GILL, and LLaVA show a significant influence of visual information in their output. 
This aligns with our findings discussed in Sec.~\ref{sec:exp_description}, where LLaVA consistently generates descriptions of the images present in the prompt rather than predicting the next image based on the sequence, thus ignoring the textual query in the prompt. 
In contrast, Qwen-VL and GPT-4V exhibit a more balanced approach, effectively integrating both textual and visual information in their predictions.

\section{Understanding Challenges in T2I-ICL}\label{sec:exp_difficulty}
In Sec.~\ref{sec:basic_exp}, we observe that most MLLMs still face challenges in performing T2I-ICL effectively.
In this section, our goal is to understand the main difficulties leading to this suboptimal performance in T2I-ICL. 
We hypothesize that the primary difficulties lie in (i) the complexity inherent to multimodality, and (ii) the intrinsic challenges of the image generation task itself, which might be independent of the T2I-ICL process.

To test these hypotheses, we conduct two experiments. 
To investigate the first hypothesis regarding multimodal complexity, we transform the T2I-ICL tasks into Textual ICL (T-ICL) by replacing the images in the prompts with their corresponding textual descriptions. 
This modification allows us to assess if the challenge primarily lies in the multimodal aspect. 
To explore the second hypothesis related to the inherent difficulty of image generation, we explicitly state the values of the latent variables in the prompts, asking the model directly to generate specific images. 
This approach will help determine if the difficulty is predominantly with the image generation process itself.

In our subsequent experiments, we mostly concentrate solely on SEED-LLaMA and Qwen-VL.
As previously shown, they are top-performing free models in image generation and image description generation, respectively.

\subsection{Is Multimodality a Primary Challenge in T2I-ICL?}\label{sec:ticl_micl}
In Sec.~\ref{sec:basic_exp}, we find that SEED-LLaMA and Qwen-VL, which are the top-performing free models for image generation and image description tasks, respectively, achieve only around or less than 50\% accuracy on most tasks. 
This is in contrast to the impressive results their underlying LLM demonstrates in Textual ICL (T-ICL)~\citep{touvron2023llama,qwen-language}.
In this experiment, our objective is to determine whether multimodality is the primary cause of this reduced performance, or whether MLLMs intrinsically struggle with these tasks even for T-ICL.

\paragraph{Prompt Design.} 
In this part, we evaluate SEED-LLaMA's capability in image generation and Qwen-VL's proficiency in image description generation by modifying the prompts to be entirely textual. 
We achieve this by replacing every image in the prompts with corresponding detailed descriptions, which are initially created by LLaVA and ChatGPT. 
These descriptions are then reviewed and corrected by humans to ensure their accuracy.
For example, in the first example depicted in Figure~\ref{fig:overview_data}, the image \img{red car} is replaced with a descriptive text: \textit{``The image portrays a red Volkswagen Golf R, a compact sports car, stationed on a wet road under a dark sky, with its vivid red color prominently contrasting the background.''}
Furthermore, to guide SEED-LLaMA in generating images rather than their descriptions, we append the following instruction at the beginning of the prompt: \textit{``We provide a few examples, each with an input, and an output of the image description. Based on the examples, predict the next image description and visualize it.'' }
Similarly, for Qwen-VL, we include an instruction: \textit{``We provide a few examples, each with an input, and an output of the image description. Based on the examples, predict the next image description.''}

\begin{table*}[!htb]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c}
        \toprule
        \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Shot}} & \multirow{2}{*}{\textbf{Method}} & \multicolumn{5}{c|}{\textbf{Object-Inference Task}} & \multicolumn{5}{c}{\textbf{Attribute-Inference Task}}  \\ \cmidrule{4-13} 
        & & & Color-I & Background-I & Style-I & Action-I & Texture-I & Color-II & Background-II & Style-II & Action-II & Texture-II \\ 
        \midrule
        \multirow{4}{*}{SEED-LLaMA} & \multirow{2}{*}{2} & T2I-ICL & \underline{\textbf{.680}} & .348 & .203 & .182 & .196 & .287 & \underline{\textbf{.467}} & \underline{\textbf{.297}} & \underline{\textbf{.261}} & .163 \\
         & & T-ICL & .614 & \textbf{.380} & \textbf{.246} & \textbf{.279} & \textbf{.265} & \textbf{.531} & .315 & .206 & .184 & \textbf{.192} \\ \cmidrule{2-13} 
         & \multirow{2}{*}{4} & T2I-ICL & .482 & .211 & .141 & .053 & .122 & .252 & .076 & .268 & \textbf{.207} & .105 \\
         & & T-ICL & \textbf{.584} & \underline{\textbf{.404}} & \underline{\textbf{.289}} & \underline{\textbf{.317}} & \underline{\textbf{.276}} & \underline{\textbf{.667}} & \textbf{.343} & \textbf{.266} & .195 & \underline{\textbf{.228}}  \\ \midrule
        \multirow{4}{*}{Qwen-VL} & \multirow{2}{*}{2} & T2I-ICL & .475 & .313 & .378 & .464 & .338 & \textbf{.457} & .379 & .258 & .388 & .316 \\
         & & T-ICL & \textbf{.854} & \textbf{.822} & \textbf{.692} & \textbf{.892} & \textbf{.679} & .272 & \textbf{.409} & \textbf{.559} & \textbf{.428} & \textbf{.431} \\ \cmidrule{2-13} 
         & \multirow{2}{*}{4} & T2I-ICL & .560 & .459 & .571 & .679 & .454 & .568 & .364 & .341 & .546 & .434 \\
         & & T-ICL & \underline{\textbf{.973}} & \underline{\textbf{.851}} & \underline{\textbf{.857}} & \underline{\textbf{.972}} & \underline{\textbf{.890}} & \underline{\textbf{.740}} & \underline{\textbf{.805}} & \underline{\textbf{.793}} & \underline{\textbf{.719}} & \underline{\textbf{.827}} \\ 
        \bottomrule
    \end{tabular}
    }
    \caption{
    \textbf{Comparison of Text-to-Image ICL (T2I-ICL) versus Textual ICL (T-ICL) accuracy on our dataset.}
    To perform T-ICL on our dataset, we replace all images in the prompts with their corresponding detailed descriptions.
    Underlined numbers indicate the highest accuracy achieved for each model and task across various shot numbers, while bold numbers indicate the highest accuracy for each specific combination of model, task, and shot count.
    In this experiment, we focus on two MLLMs: SEED-LLaMA, which is used for image generation, and Qwen-VL, utilized for generating image descriptions.
    MLLMs demonstrate notably superior performance in T-ICL compared to T2I-ICL, particularly in the 4-shot scenario. 
    }
    \label{tab:micl_ticl}
\end{table*}

\paragraph{Results.}
The results are reported in Table~\ref{tab:micl_ticl}. 
For 2-shot cases, SEED-LLaMA exhibits similar accuracies in both T2I-ICL and T-ICL, but in 4-shot instances, T-ICL surpasses T2I-ICL in 9 out of 10 tasks. 
The disparity is even more evident for Qwen-VL; under T-ICL, it significantly outperforms T2I-ICL, especially in 4-shot situations, achieving 97.3\% and 97.2\% accuracies in Color-I and Action-I tasks, respectively, and over 70\% accuracy in other tasks. 
In contrast, T2I-ICL's accuracy stays around or under 50\%. 
These findings confirm our first hypothesis, indicating that multimodality is the primary challenge in T2I-ICL. 

\subsection{Is the Image Generation a Primary Challenge in T2I-ICL?}
To verify the second hypothesis, that image generation itself presents a primary challenge in T2I-ICL, we conduct an experiment with 0, 2, and 4-shot image generation tasks, with textual inputs updated as precise labels.
For example, in the initial scenario from Figure~\ref{fig:overview_data}, the terms ``White,'' ``Blue,'' and ``Red'' are updated to ``White car,'' ``Blue car,'' and ``Red car,'' respectively. 
For this experiment, we exclude Qwen-VL as it does not generate images.
Consequently, we solely focus on SEED-LLaMA.

\begin{table*}[!htb]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c}
        \toprule
         \multirow{2}{*}{\textbf{Shot}} & \multirow{2}{*}{\begin{tabular}{c}
            \textbf{Precise}\\
            \textbf{Textual Inputs}
         \end{tabular}} & \multicolumn{5}{c|}{\textbf{Object-Inference Task}} & \multicolumn{5}{c}{\textbf{Attribute-Inference Task}}  \\ \cmidrule{3-12} 
        & & Color-I & Background-I & Style-I & Action-I & Texture-I & Color-II & Background-II & Style-II & Action-II & Texture-II \\ 
        \midrule
        0 & \cmark & .730 & \underline{.456} & \underline{.356} & \underline{.264} & .275 & .582 & .314 & .298 & .207 & \underline{.286} \\ \midrule
         \multirow{2}{*}{2} & \xmark & .680 & .348 & .203 & .182 & .196 & .287 & .467 & .297 & .261 & .163 \\
          & \cmark & \underline{\textbf{.801}} & \textbf{.409} & \textbf{.241} & \textbf{.192} & \underline{\textbf{.326}} & \textbf{.385} & \underline{\textbf{.485}} & \underline{\textbf{.393}} & \underline{\textbf{.317}} & \textbf{.268} \\ \midrule
          \multirow{2}{*}{4} & \xmark & .482 & .211 & .141 & .053 & .122 & .252 & .076 & .268 & .207 & .105 \\
          & \cmark & \textbf{.669} & \textbf{.318} & \textbf{.284} & \textbf{.161} & \textbf{.286} & \underline{\textbf{.608}} & \textbf{.441} & \textbf{.299} & \textbf{.278} & \textbf{.248} \\ 
        \bottomrule
    \end{tabular}
    }
    \caption{
        \textbf{Accuracy comparison of SEED-LLaMA, with or without providing precise textual inputs.}
        Bold numbers represent the highest accuracy for each task and shot count, comparing scenarios with and without descriptive textual inputs. 
        Underlined numbers indicate the highest accuracy for each task across various shots.
        The results illustrate that T2I-ICL with precise textual inputs that reveal latent variables, consistently surpasses scenarios without such inputs. 
    }
    \label{tab:descriptive}
\end{table*}

\paragraph{Results.}
Table~\ref{tab:descriptive} presents a comparative analysis of SEED-LLaMA's performance in T2I-ICL, both with and without the inclusion of precise textual inputs. 
Our findings indicate that in scenarios with both 2 and 4 shots, the presence of precise textual inputs leads to significantly higher accuracy in image generation compared to when these inputs are absent. 
However, it is important to note that adding more demonstrations does not necessarily translate to increased accuracy when using precise textual inputs. 
Furthermore, our analysis reveals that the performance of SEED-LLaMA, even with precise textual inputs, maintains a similar relative performance across different tasks to scenarios without these inputs. 
To be more specific, the accuracies attained by SEED-LLaMA remain below 50\% in most scenarios. 
This indicates that the task of image generation itself poses a significant challenge for current MLLMs, contributing to their underperformance on the \ours{} dataset.

\section{Enhancing MLLMs' T2I-ICL Capabilities}\label{sec:exp_enhancing}

In the previous sections, we observed the suboptimal performance of MLLMs in executing T2I-ICL and investigated the primary challenges involved. 
This section delves into exploring techniques that could potentially enhance the performance of MLLMs in T2I-ICL.

\subsection{Fine-tuning MLLMs on \ours{}}\label{sec:ft}
Building on the work of \citet{min2022metaicl}, which demonstrates that tuning models on a collection of ICL tasks enables them to learn new tasks in context at test time, we explore the impact of this approach on text-to-image generation.
We focus solely on Qwen-VL for this investigation.
Consequently, we compare the T2I-ICL performance of the pretrained-only version of Qwen-VL with the variant that is fine-tuned on our dataset.

\paragraph{Training and Test Sets.} 
The training and test sets are constructed by splitting the predefined lists of text inputs and latent variables (from Table~\ref{tab:datasets}, denoted as $\gX$ and $\Theta$) into training ($\gX_{\text{train}}$, $\Theta_{\text{train}}$) and testing ($\gX_{\text{test}}$, $\Theta_{\text{test}}$) subsets for each task, in a 1:1 ratio.
Therefore, all the in-context demonstrations and textual queries in the test sets are unseen from the training set.
For the training set, we create the dataset by considering all possible combinations and sequences of text inputs from $\gX_{\text{train}}$ and latent variables $\Theta_{\text{train}}$ across all tasks. 
We fine-tune Qwen-VL on this unified training set containing the prompts from all tasks. 
For the testing set, we generate 250 prompts for each shot across various tasks.
Each prompt is obtained by randomly sampling $\theta \in \Theta_{\text{test}}$ and $(x_n)_{n=1}^{N+1} \in \gX_{\text{test}}^{N+1}$, which are then paired with the corresponding collected images $(y_n)_{n=1}^N$, where $y_n\sim f_{\theta}(x_n)$. 
This process results in $N$ in-context demonstrations $(x_n, y_n)_{n=1}^N$ and a single textual query $x_{N+1}$.

\begin{table*}[!htbp]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c}
        \toprule
        \multirow{2}{*}{\textbf{Shot}} & \multirow{2}{*}{\textbf{Method}} & \multicolumn{5}{c|}{\textbf{Object-Inference Task}} & \multicolumn{5}{c}{\textbf{Attribute-Inference Task}}  \\ \cmidrule{3-12} 
        & & Color-I & Background-I & Style-I & Action-I & Texture-I & Color-II & Background-II & Style-II & Action-II & Texture-II \\ 
        \midrule
        \multirow{2}{*}{2} & T2I-ICL & .540 & .236 & \textbf{.248} & .412 & .372 & .276 & .244  & .112 & .232 & .224 \\
         & FT + T2I-ICL & \textbf{.852} & \underline{\textbf{.744}} & .212 & \underline{\textbf{.856}} & \textbf{.532} & \textbf{.516} & \textbf{.344} & \textbf{.148} & \textbf{.520} & \textbf{.284} \\ \midrule
         \multirow{2}{*}{4} & T2I-ICL & .680 & .492 & \underline{\textbf{.448}} & .228 & .556 & .512 & \underline{\textbf{.448}} & \underline{\textbf{.240}} & .320 & .420 \\
         & FT + T2I-ICL & \underline{\textbf{.876}} & \textbf{.604} & .216 & \textbf{.812} & \underline{\textbf{.588}} & \underline{\textbf{.696}} & .308 & .088 & \underline{\textbf{.656}} & \underline{\textbf{.480}} \\ 
        \bottomrule
    \end{tabular}
    }
    \caption{
    \textbf{T2I-ICL accuracy comparison of pretrained-only versus fine-tuned (FT) Qwen-VL.}
    Underlined numbers denote the highest performance achieved across different methods and shots for each task, while bold numbers indicate the top performance for each shot across various methods within their tasks.
    Utilizing distinct training and test sets, each with unique prompts featuring different objects and attributes, we observe that Qwen-VL, when fine-tuned on the training dataset, outperforms its pretrained-only counterpart for each shot on most of the tasks. 
    This suggests that fine-tuning with a specialized T2I-ICL dataset can enhance T2I-ICL inference capabilities.
    }
    \label{tab:ft}
\end{table*}

\paragraph{Results.} 
We fine-tune two instances of Qwen-VL, one on a 2-shot dataset and the other on a 4-shot dataset, and then compare their performances with their non-fine-tuned counterparts on the T2I-ICL test set. 
In particular, we use LoRA~\cite{hu2021lora} to update the Qwen-VL with a rank of 64, a weight decay of 0.1, and a warm-up ratio of 0.01 for 5 epochs.
The results are summarized in Table~\ref{tab:ft}. 
The results indicate a significant improvement in Qwen-VL's T2I-ICL performance post fine-tuning. 
Specifically, the fine-tuned model surpasses the original, pretrained model in nine out of ten tasks in the 2-shot scenario and in seven out of ten tasks in the 4-shot scenario.
This suggests that fine-tuning MLLMs on a T2I-ICL dataset enhances the general T2I-ICL capability of MLLMs.

\subsection{Intergrating Chain-of-Thought with T2I-ICL}\label{sec:cot}
Another widely utilized method in prompt engineering is Chain-of-Thought (CoT)~\citep{wei2022chain}. 
This approach involves incorporating a simple instruction, such as ``let's think step by step,'' prompting the model to sequentially generate concise sentences that outline the reasoning process, commonly referred to as reasoning chains or rationales. 
The chains are subsequently embedded into the subsequent prompt to obtain the final answer.
CoT has been particularly effective in enhancing performance, especially for complex reasoning tasks, when applied to large-scale models~\citep{wei2022chain}. 
In our experiment, we investigate the impact of integrating CoT on the T2I-ICL performance of MLLMs.

\paragraph{Prompt Design.}
We employ a two-step inference process utilizing two distinct prompts. 
The initial prompt builds upon the default examples showcased in Figure~\ref{fig:overview_data}. 
To this, we prepend the statement, \textit{``We provide a few examples, each of which is an input-output pair where the output is a description of the image associated with the input. Based on the examples, the task is to predict the next image description.$\backslash$n$\backslash$n$\backslash$n'' }
This is placed at the beginning of the prompt. 
Additionally, we append, \textit{``$\backslash$n$\backslash$n$\backslash$n Before predicting the next image, let's first think step by step and analyze the relationship between the text input and image output in each example.$\backslash$n$\backslash$n$\backslash$n''} to the end of the prompt.

Following the MLLMs' responses, the second prompt comes into play. 
It includes the first prompt and the MLLM's response as part of the new prompt and extends it with, \textit{``$\backslash$n$\backslash$n$\backslash$n Based on the analysis, please generate the next image for the request `red: ' ''} for the image generation scenario, and \textit{``$\backslash$n$\backslash$n$\backslash$n Based on the analysis, please describe what the next image should look like for the request `red: ' ''} for the image description generation scenario when the textual query is `red.' 
In each case, `red' is replaced with the respective textual query according to different prompts.

\begin{table*}[!htb]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c}
        \toprule
        \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Shot}} & \multirow{2}{*}{\textbf{Method}} & \multicolumn{5}{c|}{\textbf{Object-Inference Task}} & \multicolumn{5}{c}{\textbf{Attribute-Inference Task}}  \\ \cmidrule{4-13} 
        & & & Color-I & Background-I & Style-I & Action-I & Texture-I & Color-II & Background-II & Style-II & Action-II & Texture-II \\ 
        \midrule
        \multirow{4}{*}{SEED-LLaMA} & \multirow{2}{*}{2} & T2I-ICL & .680 & \textbf{.348} & .203 & \textbf{.182} & .196 & \textbf{.287} & \underline{\textbf{.467}} & \textbf{.297} & .261 & \textbf{.163} \\
         & & CoT + T2I-ICL & \underline{\textbf{.781}} & .179 & \textbf{.206} & .167 & \underline{\textbf{.222}} & .179 & .389 & .195 & \underline{\textbf{.300}} & .154 \\ \cmidrule{2-13} 
         & \multirow{2}{*}{4} & T2I-ICL & .482 & .211 & .141 & .053 & .122 & .252 & .076 & .268 & .207 & .105 \\
         & & CoT + T2I-ICL & \textbf{.650} & \underline{\textbf{.353}} & \underline{\textbf{.244}}  & \underline{\textbf{.242}} & \textbf{.208} & \underline{\textbf{.303}} & \textbf{.370} & \underline{\textbf{.335}} & \textbf{.241} & \underline{\textbf{.171}} \\ \midrule
        \multirow{4}{*}{Qwen-VL} & \multirow{2}{*}{2} & T2I-ICL & \textbf{.475} & .313 & .378 & \textbf{.464} & .338 & \textbf{.457} & \textbf{.379} & .258 & \textbf{.388} & \textbf{.316} \\
         & & CoT + T2I-ICL & .281 & \underline{\textbf{.494}} & \textbf{.387} & .217 & \textbf{.363} & .150 & .349 & \textbf{.260} & .176 & .181 \\ \cmidrule{2-13} 
         & \multirow{2}{*}{4} & T2I-ICL & \underline{\textbf{.560}} & \textbf{.459} & \underline{\textbf{.571}} & \underline{\textbf{.679}} & .454 & \underline{\textbf{.568}} & .364 & .341 & \underline{\textbf{.546}} & \underline{\textbf{.434}} \\
         & & CoT + T2I-ICL & .548 & .379 & .274 & .404 & \underline{\textbf{.573}} & .207 & \underline{\textbf{.690}} & \underline{\textbf{.409}} & .424 & .340 \\ 
        \bottomrule
    \end{tabular}
    }
    \caption{
    \textbf{Assessing the impact of Chain-of-Thought (CoT) prompting on T2I-ICL.}
    The evaluation metric is accuracy, with the numbers in bold highlighting the highest accuracy achieved for each model, number of shots, and task, and underlined numbers indicate the highest accuracy achieved for each model and task across different numbers of shots.
    In this experiment, we evaluate two MLLMs: SEED-LLaMA for image generation and Qwen-VL for image description generation.
    Our findings reveal that in 2-shot scenarios, the enhancement offered by CoT is ambiguous for both models. 
    However, in 4-shot instances, CoT markedly enhances the performance of SEED-LLaMA, while it shows no benefit for Qwen-VL.
    }
    \label{tab:cot}
\end{table*}

\paragraph{Results.} 
The results are reported in Table~\ref{tab:cot}. 
With the integration of CoT, SEED-LLaMA shows significant improvement in T2I-ICL performance across all ten tasks in the 4-shot scenario. 
However, in the 2-shot case, the benefits of CoT are less evident, with performance similar to standard T2I-ICL without CoT.
Conversely, for Qwen-VL, no concrete evidence suggests that CoT enhances its T2I-ICL performance. 
In fact, we find that Qwen-VL often avoids providing definitive answers in the second step of making predictions, and responds with general statements like \textit{``Given the request `black:', we can infer that the image output should be related to a black object or theme. However, without more specific information, it's difficult to determine the exact relationship between the text input and image output. Without additional context, it's impossible to accurately predict the next image.''}
Therefore, in many instances, standard T2I-ICL without CoT appears to outperform the version integrated with CoT for Qwen-VL.
Exploring additional prompt engineering methods such as self-consistency sampling~\citep{wang2023selfconsistency} or Tree-of-Thought~\citep{yao2023tot} to elicit more concrete responses from Qwen-VL is a possibility.
Specifically, self-consistency sampling involves generating multiple outputs at a non-zero temperature setting and selecting the most appropriate one from these options. 
On the other hand, Tree-of-Thought expands upon CoT by considering multiple lines of reasoning at each step.
However, such investigations fall outside the scope of this paper, and we identify it as one of the interesting future directions. 
For further insight, examples of prompts along with the reasoning and responses from both SEED-LLaMA and Qwen-VL are provided in Sec.~\ref{app:cot} for reference.

\subsection{Articulating the Text-to-Image Relationship in Prompts}\label{sec:exact_instruction}
In our dataset, the goal is to check if the MLLMs are able to learn the mapping from the textual input and the visual output based on the in-context demonstrations. 
In this experiment, we investigate the performance of MLLMs on T2I-ICL if we explicitly write down this relationship in the text prompt. 
For instance, for the Color-I task, we directly add the following sentence to the beginning of the prompt: \textit{``Please identify the common main object in the images, and generate another image of this object in the requested color.''} 
The detailed prompts for all tasks are provided in Sec.~\ref{app:prompt_explicit_instruction}. 

\begin{table*}[!htbp]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c}
        \toprule
        \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Shot}} & \multirow{2}{*}{\begin{tabular}{c}
            \textbf{Explicit}  \\
            \textbf{Instruction} 
        \end{tabular}} & \multicolumn{5}{c|}{\textbf{Object-Inference Task}} & \multicolumn{5}{c}{\textbf{Attribute-Inference Task}}  \\ \cmidrule{4-13} 
        & & & Color-I & Background-I & Style-I & Action-I & Texture-I & Color-II & Background-II & Style-II & Action-II & Texture-II \\ 
        \midrule
        \multirow{4}{*}{SEED-LLaMA} & \multirow{2}{*}{2} & \xmark & .680 & .348 & .203 & .182 & .196 & \textbf{.287} & \textbf{.467} & .297 & \textbf{.261} & .163 \\
         & & \cmark & \textbf{.779} & \textbf{.391} & \textbf{.231} & \textbf{.301} & \textbf{.270} & .257 & .446 & \textbf{.350} & .249 & \textbf{.185} \\ \cmidrule{2-13} 
         & \multirow{2}{*}{4} & \xmark & .482 & .211 & .141 & .053 & .122 & .252 & .076 & .268 & .207 & .105 \\
         & & \cmark & \underline{\textbf{.832}} & \underline{\textbf{.408}} & \underline{\textbf{.281}} & \underline{\textbf{.318}} & \underline{\textbf{.322}} & \underline{\textbf{.388}} & \underline{\textbf{.483}} & \underline{\textbf{.406}} & \underline{\textbf{.268}} & \underline{\textbf{.228}} \\ \midrule
        \multirow{4}{*}{Qwen-VL} & \multirow{2}{*}{2} & \xmark & \textbf{.475} & .313 & \textbf{.378} & .464 & \textbf{.338} & \textbf{.457} & .379 & .258 & .388 & .316 \\
         & & \cmark & .407 & \underline{\textbf{.496}} & .240 & \textbf{.516} & .300 & .240 & \underline{\textbf{.697}} & \textbf{.317} & \underline{\textbf{.600}} & \textbf{.373} \\ \cmidrule{2-13} 
         & \multirow{2}{*}{4} & \xmark & \underline{\textbf{.560}} & \textbf{.459} & \underline{\textbf{.571}} & \underline{\textbf{.679}} & \underline{\textbf{.454}} & \underline{\textbf{.568}} & .364 & \underline{\textbf{.341}} & \textbf{.546} & \underline{\textbf{.434}} \\
         & & \cmark & .315 & .291 & .341 & .475 & .473 & .277 & \textbf{.591} & .317 & .527 & .404 \\ 
        \bottomrule
    \end{tabular}
    }
    \caption{
        \textbf{Effect of explicit instruction on T2I-ICL performance of MLLMs: articulating the text-to-image relationship in prompts.}
        The evaluation metric is accuracy, where underlined numbers denote the highest accuracy achieved by each model and task across varying shot numbers, and bold numbers represent the top accuracy for each specific combination of model, task, and shot count.
        This evaluation focuses on SEED-LLaMA for image generation and Qwen-VL for image description generation.
        We find that explicit instructions significantly enhance the T2I-ICL capability of SEED-LaMA, especially in the 4-shot scenario.
        However, for Qwen-VL, explicit instructions do not show similar performance gains.
    }
    \label{tab:instruction}
\end{table*}

\paragraph{Results.} 
We present the experiment results in Table~\ref{tab:instruction}. 
Results show that SEED-LLaMA's performance significantly improves with explicit instructions, surpassing its performance in T2I-ICL without instructions for seven out of ten tasks in the 2-shot cases and all tasks in the 4-shot cases.
Notably, in the 4-shot case for the Color-I task, SEED-LLaMA achieves a high accuracy of 83.2\% with explicit instructions, compared to only 48.2\% without them.
Furthermore, the performance of T2I-ICL with explicit instructions improves when moving from 2-shot to 4-shot scenarios, in contrast to the situation without explicit instructions where SEED-LLaMA's T2I-ICL performance declines as the number of demonstrations increases from 2 to 4.
In contrast, Qwen-VL does not show comparable improvements, owing to reasons similar to those discussed in Sec.~\ref{sec:cot},  including the generation of irrelevant responses like \textit{``Received.''}


\section{Conclusion}
In this work, we identify an important yet underexplored problem — T2I-ICL, and explore the capability of MLLMs to solve it.
To facilitate this investigation, we introduce \ours{}, a comprehensive benchmark dataset encompassing ten tasks. 
Our experimental evaluation of MLLMs on this dataset reveals that while many MLLMs have difficulty in effectively learning from in-context demonstrations during text-to-image generation, a few MLLMs, such as GPT-4V, Qwen-VL, and SEED-LaMA, show comparatively reasonable performance.
Through further studies on free top-performing models SEED-LLaMA and Qwen-VL for both image and image description generation, we identify two key challenges in T2I-ICL: 
(i) the integration and understanding of multimodal information, evidenced by superior results achieved with textual ICL for the same tasks; and 
(ii, particularly for image generation models) the actual process of image creation, as even straightforward image requests with clear descriptions often yield suboptimal performances.

To improve MLLMs' performance in T2I-ICL, we carry out additional experimental studies. 
These studies suggest that fine-tuning can substantially enhance T2I-ICL capabilities.
Meanwhile, it is worth noting that in our dataset, we intentionally exclude explicit task descriptions to assess whether MLLMs can autonomously adapt to tasks based solely on in-context demonstrations alone. 
Nevertheless, providing clearer task instructions might be a promising strategy for enhancing T2I-ICL performance. 
This also holds for CoT prompting.
While these strategies notably improve SEED-LLaMA's performance in the experiment, they do not have a similar impact on Qwen-VL, suggesting that these prompt engineering techniques might need to be combined with others to achieve universal effectiveness.



\section{Limitations and Future Works}
While our study is an early attempt to explore the T2I-ICL benchmark dataset, many interesting questions remain open. 


\paragraph{Impact of Demonstration Selection on T2I-ICL Performance.}
Existing research in textual ICL has consistently demonstrated that the choice of demonstrations significantly influences ICL performances~\citep{liu2022what,su2023selective,rubin2022learning,zhang2022active}.
In our study, we only employ random sampling to select in-context demonstrations.
This opens an interesting question: to what extent does the selection of demonstrations affect T2I-ICL performance?
Moreover, our evaluation primarily assesses whether MLLMs can accurately generate images with the current content, without a specific focus on the quality of these images. 
Another natural question arises: how significantly does the quality of images used in demonstrations influence the overall quality of the generated image output? 

\paragraph{Prompt Engineering Techniques for MLLMs.}
As discussed in Sec.~\ref{sec:cot}, CoT demonstrates significant improvements in T2I-ICL performance for SEED-LLaMA.
However, the prompt sensitivity of models like Qwen-VL poses a challenge, as they tend to provide non-committal responses such as, \textit{``Without additional context, it's impossible to accurately predict the next image.''}
This issue underscores the necessity of implementing more advanced prompt engineering techniques, including methods like Tree-of-Thought and self-consistency sampling, to address these limitations. 

Once such issues are resolved, another interesting question arises: Is it feasible to enhance existing prompt engineering techniques with multimodal capabilities?
For instance, while Sec.~\ref{sec:cot} focuses on prompting MLLM to perform CoT through textual analysis (as further exemplified in Sec.~\ref{app:cot}), expanding this approach to a multimodal CoT that integrates both textual analysis and image grounding could potentially yield better performance. 
These open questions are identified as interesting future directions. 

\paragraph{T2I-ICL for Image Editing.}
One notable absence in our dataset is tasks related to image editing. 
For instance, in the Color-I task, the goal is to generate an image of a car in a color specified by the text query.
In our evaluation, the car type and background in both the example images from the prompt and the newly generated image may differ.
However, there is a growing need for image editing applications where the task is to alter specific attributes (\eg, the color of a car) in an otherwise unchanged image. 
For such tasks, selecting images that strictly adhere to the given criteria (identical images with only specific attributes or objects altered), coupled with the development of sophisticated metrics, is critical to assess these more complex challenges effectively.

\paragraph{Exploring a Wider Range of Themes.}
Our dataset primarily assesses MLLMs on elementary themes, incorporating a specific range of objects and attributes within narrowly defined categories. 
For instance, in the style task, we consider styles such as watercolor, sketch, pixel art, origami, and others. 
Nonetheless, the realm of styles in real-world applications is far more intricate and varied, extending to include oil painting, rococo, steampunk, and beyond. 
Additionally, our dataset encompasses a limited set of themes.
There are also many other interesting themes such as counting. 
While it serves to test basic capabilities in T2I-ICL, a more comprehensive dataset, covering a broader spectrum of themes and a finer list of objects and attributes, will be crucial for evaluating more advanced model capabilities.
In this scenario, the evaluation methodology may require refinement to more accurately identify the more fine-grained attributes and objects.


==> math_commands2.tex <==

\usepackage{amsmath,amsfonts,bm}

\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

\newcommand{\newterm}[1]{{\bf #1}}


\def\figref#1{figure~\ref{#1}}
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
\def\secref#1{section~\ref{#1}}
\def\Secref#1{Section~\ref{#1}}
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
\def\eqref#1{equation~\ref{#1}}
\def\Eqref#1{Equation~\ref{#1}}
\def\plaineqref#1{\ref{#1}}
\def\chapref#1{chapter~\ref{#1}}
\def\Chapref#1{Chapter~\ref{#1}}
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
\def\algref#1{algorithm~\ref{#1}}
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
\def\partref#1{part~\ref{#1}}
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

\newcommand{\pdata}{p_{\rm{data}}}
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} %

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} %

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tex/figures/fig_comparison.tex <==
\tikzset{
  pics/title/.style args={#1,#2,#3}{
     code={
        \path [rounded corners, fill=mycolor2] (-2.6,2.1) rectangle ++(2,0.6) node[pos=.5,text=white] {\normalsize Latent Var.};

        \path [rounded corners, fill=mycolor2] (0,2.1) rectangle ++(10.2,0.6) node[pos=.5,text=white] {\normalsize Input};
        
        \path [rounded corners, fill=mycolor2] (10.5,2.1) rectangle ++(2.8,0.6) node[pos=.5,text=white] {\normalsize #1};
        \path [rounded corners, fill=mycolor2] (13.5,2.1) rectangle ++(2.8,0.6) node[pos=.5,text=white] {\normalsize #2};
        \path [rounded corners, fill=mycolor2] (16.5,2.1) rectangle ++(2.8,0.6) node[pos=.5,text=white] {\normalsize #3};
        
     }
  }
}

\tikzset{
  pics/cell/.style args={#1,#2}{
     code={
        \draw [rounded corners, fill=mycolor1] (0,0) rectangle ++(2.8,2);

        \begin{scope}
        \clip (0.6,0.2) rectangle ++(1.6,1.6) ;
        \node at (1.4,1) {\includegraphics[height=1.6cm]{#2}}; 
        \end{scope}
        
     }
  }
}

\tikzset{
  pics/row1/.style args={#1,#2,#3,#4,#5}{
     code={
        \draw [rounded corners, fill=mycolor1] (-2.6,0) rectangle ++(2,2) node[pos=.5] {\normalsize #1};
        \draw [rounded corners, fill=mycolor1] (0,0) rectangle ++(10.2,2);

        \node at (1,1) {\normalsize #2: };
        \node at (5,1) {\normalsize #3: };
        \node at (9,1) {\normalsize #4: };

        \begin{scope}
        \clip (2.2,0.2) rectangle ++(1.6,1.6) ;
        \node at (3,1) {\includegraphics[height=1.6cm]{tex/datasets/#2_#1.jpg}}; 
        \end{scope}

        \begin{scope}
        \clip (6.2,0.2) rectangle ++(1.6,1.6) ;
        \node at (7,1) {\includegraphics[height=1.6cm]{tex/datasets/#3_#1.jpg}}; 
        \end{scope}
        
        \draw (10.5,0) pic{cell={Emu,figures/results/emu_#5_#1_#2_#3_#4.jpg}};
        \draw (13.5,0) pic{cell={GILL,figures/results/gill_#5_#1_#2_#3_#4.jpg}};
        \draw (16.5,0) pic{cell={SEED-LLaMA,figures/results/seed_#5_#1_#2_#3_#4.jpg}};
        
     }
  }
}




        
        

\tikzset{
  pics/row2/.style args={#1,#2,#3,#4,#5}{
     code={
        \draw [rounded corners, fill=mycolor1] (-2.6,0) rectangle ++(2,2) node[pos=.5] {\normalsize #1};
        \draw [rounded corners, fill=mycolor1] (0,0) rectangle ++(10.2,2);

        \node at (1,1) {\normalsize #2: };
        \node at (5,1) {\normalsize #3: };
        \node at (9,1) {\normalsize #4: };

        \begin{scope}
        \clip (2.2,0.2) rectangle ++(1.6,1.6) ;
        \node at (3,1) {\includegraphics[height=1.6cm]{tex/datasets/#1_#2.jpg}}; 
        \end{scope}


        \begin{scope}
        \clip (6.2,0.2) rectangle ++(1.6,1.6) ;
        \node at (7,1) {\includegraphics[height=1.6cm]{tex/datasets/#1_#3.jpg}}; 
        \end{scope}
        
        \draw (10.5,0) pic{cell={Emu,figures/results/emu_#5_#1_#2_#3_#4.jpg}};
        \draw (13.5,0) pic{cell={GILL,figures/results/gill_#5_#1_#2_#3_#4.jpg}};       
        \draw (16.5,0) pic{cell={SEED-LLaMA,figures/results/seed_#5_#1_#2_#3_#4.jpg}};
        
     }
  }
}


\begin{figure*}[!htb]

    \begin{subfigure}[b]{\linewidth}
        \centering
        \resizebox{\linewidth}{!}{%
            \begin{tikzpicture}
            \tikzstyle{every node}=[font=\large]
    
            \draw (0,0) pic{title={Emu,GILL,SEED-LLaMA}};
    
            \draw (0,0) pic{row1={Bag,Brown,Blue,Purple,873}};
            \draw (0,-2.1) pic{row1={Car,Brown,Purple,Orange,519}};
            \draw (0,-4.2) pic{row1={Hat,Green,Yellow,White,893}};
            \draw (0,-6.3) pic{row1={Book,Purple,White,Pink,324}};
            \draw (0,-8.4) pic{row1={Box,White,Yellow,Green,655}};
            \draw (0,-10.5) pic{row1={Leaf,Pink,Brown,Blue,445}};
    
        \end{tikzpicture}
        }
        \caption{Color-I}
    \end{subfigure}
    \begin{subfigure}[b]{\linewidth}
        \centering
        \resizebox{\linewidth}{!}{%
        \begin{tikzpicture}
        \tikzstyle{every node}=[font=\large]

        \draw (0,0) pic{title={Emu,GILL,SEED-LLaMA}};

        \draw (0,0) pic{row2={Purple,Cup,Box,Bag,753}};
        \draw (0,-2.1) pic{row2={Orange,Ball,Book,Car,307}};
        \draw (0,-4.2) pic{row2={White,Book,Leaf,Hat,893}};
        \draw (0,-6.3) pic{row2={Pink,Box,Hat,Book,199}};
        \draw (0,-8.4) pic{row2={Green,Ball,Bag,Box,71}};
        \draw (0,-10.5) pic{row2={Blue,Ball,Bag,Leaf,94}};

        \end{tikzpicture}
        }
        \caption{Color-II}
    \end{subfigure}
    \caption{Examples of prompts and corresponding images generated by MLLMs for tasks within the Color theme.}
    \label{fig:example_image_color}
\end{figure*}

\begin{figure*}[!htb]

    \begin{subfigure}[b]{\linewidth}
        \centering
        \resizebox{\linewidth}{!}{%
            \begin{tikzpicture}
            \tikzstyle{every node}=[font=\large]
    
            \draw (0,0) pic{title={Emu,GILL,SEED-LLaMA}};
    
            \draw (0,0) pic{row1={Bird,Seafloor,Beach,Waterfall,25}};
            \draw (0,-2.1) pic{row1={Lion,Gym,Seafloor,Beach,152}};
            \draw (0,-4.2) pic{row1={Tiger,Desert,Park,Glacier,954}};
            \draw (0,-6.3) pic{row1={Monkey,Waterfall,Cave,Desert,633}};
            \draw (0,-8.4) pic{row1={Zebra,Beach,Waterfall,Cave,760}};
            \draw (0,-10.5) pic{row1={Cat,Waterfall,Beach,Gym,13}};
    
        \end{tikzpicture}
        }
        \caption{Background-I}
    \end{subfigure}
    \begin{subfigure}[b]{\linewidth}
        \centering
        \resizebox{\linewidth}{!}{%
        \begin{tikzpicture}
        \tikzstyle{every node}=[font=\large]

        \draw (0,0) pic{title={Emu,GILL,SEED-LLaMA}};

        \draw (0,0) pic{row2={Waterfall,Tiger,Monkey,Bird,2}};
        \draw (0,-2.1) pic{row2={Beach,Monkey,Dog,Lion,278}};
        \draw (0,-4.2) pic{row2={Glacier,Monkey,Lion,Tiger,852}};
        \draw (0,-6.3) pic{row2={Desert,Lion,Dog,Monkey,882}};
        \draw (0,-8.4) pic{row2={Cave,Cow,Cat,Zebra,94}};
        \draw (0,-10.5) pic{row2={Gym,Dog,Monkey,Cat,234}};
        \end{tikzpicture}
        }
        \caption{Background-II}
    \end{subfigure}
    \caption{Examples of prompts and corresponding images generated by MLLMs for tasks within the Background theme.}
    \label{fig:example_image_background}
\end{figure*}

\begin{figure*}[!htb]
    \begin{subfigure}[b]{\linewidth}
        \centering
        \resizebox{\linewidth}{!}{%
            \begin{tikzpicture}
            \tikzstyle{every node}=[font=\large]
    
            \draw (0,0) pic{title={Emu,GILL,SEED-LLaMA}};
    
            \draw (0,0) pic{row1={Cup,Lego,Origami,Sketch,54}};
            \draw (0,-2.1) pic{row1={Chair,Icon,Pixel,Watercolor,350}};
            \draw (0,-4.2) pic{row1={Book,Sketch,Lego,Old,2}};
            \draw (0,-6.3) pic{row1={Ball,Pixel,Sketch,Graffiti,73}};
            \draw (0,-8.4) pic{row1={Apple,Futuristic,Origami,Icon,410}};
            \draw (0,-10.5) pic{row1={Bag,Lego,Futuristic,Origami,23}};
    
        \end{tikzpicture}
        }
        \caption{Style-I}
    \end{subfigure}
    \begin{subfigure}[b]{\linewidth}
        \centering
        \resizebox{\linewidth}{!}{%
        \begin{tikzpicture}
        \tikzstyle{every node}=[font=\large]

        \draw (0,0) pic{title={Emu,GILL,SEED-LLaMA}};

        \draw (0,0) pic{row2={Sketch,Car,Apple,Cup,237}};
        \draw (0,-2.1) pic{row2={Watercolor,Cup,Apple,Chair,332}};
        \draw (0,-4.2) pic{row2={Old,Cup,Ball,Book,302}};
        \draw (0,-6.3) pic{row2={Graffiti,Bag,Hat,Ball,494}};
        \draw (0,-8.4) pic{row2={Icon,Leaf,Car,Apple,56}};
        \draw (0,-10.5) pic{row2={Origami,Book,Ball,Bag,497}};

        \end{tikzpicture}
        }
        \caption{Style-II}
    \end{subfigure}
    \caption{Examples of prompts and corresponding images generated by MLLMs for tasks within the Style theme.}
    \label{fig:example_image_style}
\end{figure*}

\begin{figure*}[!htb]
    \begin{subfigure}[b]{\linewidth}
        \centering
        \resizebox{\linewidth}{!}{%
            \begin{tikzpicture}
            \tikzstyle{every node}=[font=\large]
    
            \draw (0,0) pic{title={Emu,GILL,SEED-LLaMA}};
    
            \draw (0,0) pic{row1={Dog,Run,Drink,Swim,916}};
            \draw (0,-2.1) pic{row1={Zebra,Fly,Swim,Drink,93}};
            \draw (0,-4.2) pic{row1={Cat,Run,Cry,Eat,304}};
            \draw (0,-6.3) pic{row1={Pig,Eat,Drink,Angry,230}};
            \draw (0,-8.4) pic{row1={Sheep,Eat,Angry,Sleep,878}};
            \draw (0,-10.5) pic{row1={Lion,Eat,Cry,Run,236}};
    
        \end{tikzpicture}
        }
        \caption{Action-I}
    \end{subfigure}
    \begin{subfigure}[b]{\linewidth}
        \centering
        \resizebox{\linewidth}{!}{%
        \begin{tikzpicture}
        \tikzstyle{every node}=[font=\large]

        \draw (0,0) pic{title={Emu,GILL,SEED-LLaMA}};

        \draw (0,0) pic{row2={Swim,Monkey,Sheep,Dog,216}};
        \draw (0,-2.1) pic{row2={Drink,Cat,Sheep,Zebra,648}};
        \draw (0,-4.2) pic{row2={Eat,Bird,Pig,Cat,725}};
        \draw (0,-6.3) pic{row2={Angry,Bird,Cow,Pig,401}};
        \draw (0,-8.4) pic{row2={Sleep,Pig,Dog,Sheep,44}};
        \draw (0,-10.5) pic{row2={Run,Tiger,Pig,Lion,899}};

        \end{tikzpicture}
        }
        \caption{Action-II}
    \end{subfigure}
    \caption{Examples of prompts and corresponding images generated by MLLMs for tasks within the Action theme.}
    \label{fig:example_image_action}
\end{figure*}

\begin{figure*}[!htb]
    \begin{subfigure}[b]{\linewidth}
        \centering
        \resizebox{\linewidth}{!}{%
            \begin{tikzpicture}
            \tikzstyle{every node}=[font=\large]
    
            \draw (0,0) pic{title={Emu,GILL,SEED-LLaMA}};
    
            \draw (0,0) pic{row1={Ball,Leather,Wicker,Metal,390}};
            \draw (0,-2.1) pic{row1={Box,Metal,Sequined,Wood,364}};
            \draw (0,-4.2) pic{row1={Hat,Ceramic,Paper,Wicker,653}};
            \draw (0,-6.3) pic{row1={Bag,Ceramic,Sequined,Denim,256}};
            \draw (0,-8.4) pic{row1={Cup,Plastic,Denim,Ceramic,896}};
            \draw (0,-10.5) pic{row1={Car,Lace,Paper,Plastic,273}};
    
        \end{tikzpicture}
        }
        \caption{Texture-I}
    \end{subfigure}
    \begin{subfigure}[b]{\linewidth}
        \centering
        \resizebox{\linewidth}{!}{%
        \begin{tikzpicture}
        \tikzstyle{every node}=[font=\large]

        \draw (0,0) pic{title={Emu,GILL,SEED-LLaMA}};

        \draw (0,0) pic{row2={Metal,Bag,Hat,Ball,180}};
        \draw (0,-2.1) pic{row2={Wood,Leaf,Book,Box,88}};
        \draw (0,-4.2) pic{row2={Wicker,Ball,Cup,Hat,801}};
        \draw (0,-6.3) pic{row2={Denim,Ball,Box,Bag,481}};
        \draw (0,-8.4) pic{row2={Ceramic,Chair,Box,Cup,597}};
        \draw (0,-10.5) pic{row2={Plastic,Leaf,Ball,Car,582}};

        \end{tikzpicture}
        }
        \caption{Texture-II}
    \end{subfigure}
    \caption{Examples of prompts and corresponding images generated by MLLMs for tasks within the Texture theme.}
    \label{fig:example_image_texture}
\end{figure*}


==> tex/figures/fig_framework.tex <==
\tikzset{
  pics/myprompt3/.style args={#1,#2,#3,#4}{
     code={
        \path [rounded corners, fill=mycolor3] (0,0) rectangle ++(13.2,2.7);
        
        \draw [rounded corners, fill=mycolor1] (0,0) rectangle ++(10,2);
        \draw [rounded corners, fill=mycolor1] (10.2,0) rectangle ++(3,2) node[pos=.5] {\underline{#4 #1}};
        \node at (1,1) {#2: };
        \node at (5,1) {#3: };
        \node at (9,1) {#4: };
        
        \begin{scope}
        \clip (2.2,0.2) rectangle ++(1.6,1.6) ;
        \node at (3,1) {\includegraphics[height=1.6cm]{tex/datasets/#2_#1}}; 
        \end{scope}
        \begin{scope}
        \clip (6.2,0.2) rectangle ++(1.6,1.6) ;
        \node at (7,1) {\includegraphics[height=1.6cm]{tex/datasets/#3_#1}};
        \end{scope}

        \path [rounded corners, fill=mycolor2] (0,2.1) rectangle ++(10,0.6) node[pos=.5,text=white] {\normalsize Prompt};

        \path [rounded corners, fill=mycolor2] (10.2,2.1) rectangle ++(3,0.6) node[pos=.5,text=white] {\normalsize True label};

        \path [rounded corners, fill=mycolor3] (-1,0) rectangle ++(0.8,2.7) node[pos=.5,rotate=90] {\textbf{Example}};
        
     }
  }
}

\tikzset{
  pics/myfigure1/.style args={#1,#2,#3,#4,#5,#6}{
     code={        
        \path [rounded corners, fill=mycolor2] (0,14.2) rectangle ++(6.5,0.8) node[pos=.5,text=white] {\textbf{#5}};

        \draw [rounded corners, thick] (0,0) rectangle ++(6.5,14);
        \path [rounded corners, fill=mycolor4] (0,6.3) rectangle ++(6.5,7.7);
        \path [rounded corners, fill=mycolor5] (0,0) rectangle ++(6.5,6.3);
        

        \path [rounded corners, fill=mycolor2] (1.75,11.5) rectangle ++(3,0.6) node[pos=.5,text=white] {\normalsize Prompt};


        \draw [line width=0.07cm, -latex] (3.5,11.4) -- ++(-45:0.6cm);
        \draw [line width=0.07cm, -latex] (3,11.4) -- ++(225:0.6cm);



        \draw [line width=0.1cm,color=mycolor2,fill=white] (0.6,9.3) rectangle ++(2,1.5) node[pos=.5,text=black] {\begin{tabular}{c} MLLM A \end{tabular}};

        \draw [line width=0.1cm,color=mycolor2,fill=white] (3.9,9.3) rectangle ++(2,1.5) node[pos=.5,text=black] {\begin{tabular}{c} MLLM B \end{tabular}};

        
        \draw [line width=0.07cm, -latex] (1.6,9.1) to (1.6,8.6);
        \draw [line width=0.07cm, -latex] (4.9,9.1) to (4.9,8.6);

        \draw [rounded corners, fill=mycolor1] (0.6,6.5) rectangle ++(2,2);
        \draw [rounded corners, fill=mycolor1] (3.9,6.5) rectangle ++(2,2);

        \begin{scope}
        \clip (0.8,6.7) rectangle ++(1.6,1.6) ;
        \node at (1.6,7.5) {\includegraphics[height=1.6cm]{tex/datasets/#4_#1}}; 
        \end{scope}

        
        \begin{scope}
        \clip (4.1,6.7) rectangle ++(1.6,1.6) ;
        \node at (4.9,7.5) {\includegraphics[height=1.6cm]{figures/chair.png}}; 
        \end{scope}

        \node at (2.4,6.3) {+};
        \node at (0.8,6.3) {+};
        \node at (4.1,6.3) {+};
        \node at (5.7,6.3) {+};

        \draw [line width=0.07cm, -latex] (2.4,5.4) to (2.4,4.9);
        \draw [line width=0.07cm, -latex] (0.8,5.4) to (0.8,4.9);
        
        \draw [line width=0.07cm, -latex] (4.1,5.4) to (4.1,4.9);
        \draw [line width=0.07cm, -latex] (5.7,5.4) to (5.7,4.9);




        \draw [line width=0.1cm,color=mycolor2,fill=white] (0.5,3.3) rectangle ++(5.5,1.5) node[pos=.5,text=black] {LLaVA};


        \draw [rounded corners, fill=mycolor1] (0.2,5.5) rectangle ++(1.2,0.6) node[pos=.5,text=black] {\small{\textit{color?}}};
        \draw [rounded corners, fill=mycolor1] (1.8,5.5) rectangle ++(1.2,0.6) node[pos=.5,text=black] {\small{\textit{object?}}};

        \draw [rounded corners, fill=mycolor1] (3.5,5.5) rectangle ++(1.2,0.6) node[pos=.5,text=black] {\small{\textit{color?}}};
        \draw [rounded corners, fill=mycolor1] (5.1,5.5) rectangle ++(1.2,0.6) node[pos=.5,text=black] {\small{\textit{object?}}};


        \draw [line width=0.07cm, -latex] (2.4,3.1) to (2.4,2.6);
        \draw [line width=0.07cm, -latex] (0.8,3.1) to (0.8,2.6);
        
        \draw [line width=0.07cm, -latex] (4.1,3.1) to (4.1,2.6);
        \draw [line width=0.07cm, -latex] (5.7,3.1) to (5.7,2.6);

        \draw [rounded corners, fill=mycolor1] (0.2,1.9) rectangle ++(1.2,0.6) node[pos=.5,text=black] {\small{\textit{black}}};
        \draw [rounded corners, fill=mycolor1] (1.8,1.9) rectangle ++(1.2,0.6) node[pos=.5,text=black] {\small{\textit{chair}}};

        \draw [rounded corners, fill=mycolor1] (3.5,1.9) rectangle ++(1.2,0.6) node[pos=.5,text=black] {\small{\textit{pink}}};
        \draw [rounded corners, fill=mycolor1] (5.1,1.9) rectangle ++(1.2,0.6) node[pos=.5,text=black] {\small{\textit{chair}}};


        \node at (2.4,1.5) {\includegraphics[height=0.6cm]{figures/good.png}};
        \node at (0.8,1.5) {\includegraphics[height=0.6cm]{figures/good.png}};
        \node at (1.6,0.5) {\includegraphics[height=0.6cm]{figures/good.png}};

        \node at (5.7,1.5) {\includegraphics[height=0.6cm]{figures/good.png}};
        \node at (4.1,1.5) {\includegraphics[height=0.8cm]{figures/bad.png}};
        \node at (4.9,0.5) {\includegraphics[height=0.8cm]{figures/bad.png}};

        \draw [line width=0.07cm] (1.3,1.5) to (1.9,1.5);
        \draw [line width=0.07cm, -latex] (1.6,1.5) to (1.6,0.9);
        \draw [line width=0.07cm] (4.6,1.5) to (5.2,1.5);
        \draw [line width=0.07cm, -latex] (4.9,1.5) to (4.9,0.9);

     }
  }
}

\tikzset{
  pics/myfigure2/.style args={#1,#2,#3,#4,#5,#6}{
     code={
        \draw (0,0) pic{myfigure1={#1,#2,#3,#4,#5,#6}};
        
        \draw [rounded corners, fill=mycolor1] (0.2,12.5) rectangle ++(6.1,1.3) node[pos=.5,text=black] {\textit{\small{{\begin{tabular}{c} I will provide you with a few examples with \\ text and images. Complete the examples \\ with the description of the next image. \end{tabular}}}}};
        \node at (3.25,12.3) {+};
        
        \draw [rounded corners, fill=mycolor1] (3.9,6.5) rectangle ++(2,2) node[pos=.5,text=black] {\textit{\small{{\begin{tabular}{c} a pink chair \\ with wooden \\ legs \end{tabular}}}}};
        \draw [rounded corners, fill=mycolor1] (0.6,6.5) rectangle ++(2,2) node[pos=.5,text=black] {\textit{\small{{\begin{tabular}{c} black chair \\ on white\\ background \end{tabular}}}}};

        \path [rounded corners, fill=mycolor4] (-7.7,6.3) rectangle ++(0.8,7.7) node[pos=.5,rotate=90] {\textbf{\Large Inference Stage}};
        \path [rounded corners, fill=mycolor5] (-7.7,0) rectangle ++(0.8,6.3) node[pos=.5,rotate=90] {\textbf{\Large Evaluation Stage}};


     }
  }
}


\begin{figure}[!h]
    \centering
        \resizebox{1\linewidth}{!}{%
    \begin{tikzpicture}
        \tikzstyle{every node}=[font=\large]

        \draw (0,0) pic{myprompt3={Chair,Yellow,Pink,Black}};
        \draw (0,-15.5) pic{myfigure1={Chair,Yellow,Pink,Black,Image Generation,Emu}};
        \draw (6.7,-15.5) pic{myfigure2={Chair,Yellow,Pink,Black,Image Description Generation,GPT-4V}};

    \end{tikzpicture}
    }%
    \caption{
        \textbf{Benchmarking pipline for MLLMs in T2I-ICL with \ours{}.}
        This pipeline outlines the process to assess MLLMs in T2I-ICL. 
        Initially, we input prompts from our dataset into MLLMs capable of image generation. 
        The key step involves evaluating the generated images' alignment with the actual label, exemplified by the target label ``black chair'' in this case. 
        If the MLLM accurately interprets the text-image relationship in the provided demonstrations, it should produce an image of a ``black chair.''
        To verify this alignment, we utilize LLaVA to identify the main object and specific attributes (\eg, color) based on the task's theme. 
        We then compare LLaVA's output with the true label to determine the image's accuracy. 
        For MLLMs that do not generate images, we modify the process by instructing the MLLMs to describe the image textually, following the same evaluation criteria as in the image generation scenario. 
        The pipeline features two illustrative examples for each scenario: one where the MLLM generates a correct output and another where it produces an incorrect output.
    }
    \label{fig:framework_flow}
\end{figure}







==> tex/figures/fig_intro.tex <==
\tikzset{
  pics/myprompt3/.style args={#1}{
     code={
        
        \draw [rounded corners, fill=mycolor1] (0,0) rectangle ++(10,2);
        \draw [rounded corners, fill=mycolor1] (12,0) rectangle ++(3,2);

        \draw[ultra thick,-latex] (10.2,1) --node[pos=.5,sloped, anchor=center,above=3pt]{\normalsize #1} (11.8,1);

        \path [rounded corners, fill=mycolor2] (0,2.1) rectangle ++(10,0.6) node[pos=.5,text=white] {\normalsize Input};

        \path [rounded corners, fill=mycolor2] (12,2.1) rectangle ++(3,0.6) node[pos=.5,text=white] {\normalsize Output};
        
     }
  }
}

\begin{figure*}[!h]
\vspace{.1in}
    \centering
    \begin{minipage}[b]{0.49\linewidth}
    \begin{subfigure}[b]{\textwidth}
    \caption{Textual ICL~\citep{brown2020gpt3}}
    \label{fig:demo_text}
    \resizebox{1\textwidth}{!}{%
    \centering
    \begin{tikzpicture}
        \tikzstyle{every node}=[font=\large]

        \draw (0,0) pic{myprompt3={LLM}};
        \node at (1,1) {thanks: };
        \node at (3,1) {merci};
        \node at (5,1) {hello: };
        \node at (7,1) {bonjour};
        \node at (9,1) {mint: };
        
        \node at (13.5,1) {menthe};

    \end{tikzpicture}
    }
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}
        \caption{Visual ICL~\citep{bar2022visual}}
        \label{fig:demo_visual}
    \resizebox{1\textwidth}{!}{%
    \centering
    \begin{tikzpicture}
        \tikzstyle{every node}=[font=\large]

        \draw (0,0) pic{myprompt3={VM}};







        \begin{scope}
        \clip (0.2,0.2) rectangle ++(3.27,1.6) ;
        \node at (1.835,1) {\includegraphics[height=1.6cm]{figures/b1xy.png}};
        \end{scope}
        \begin{scope}
        \clip (4.2,0.2) rectangle ++(3.27,1.6) ;
        \node at (5.835,1) {\includegraphics[height=1.6cm]{figures/b2xy.png}}; 
        \end{scope}
        \begin{scope}
        \clip (8.2,0.2) rectangle ++(1.6,1.6) ;
        \node at (9,1) {\includegraphics[height=1.6cm]{figures/b3x-.png}}; 
        \end{scope}
        \begin{scope}
        \clip (12.7,0.2) rectangle ++(1.6,1.6) ;
        \node at (13.5,1) {\includegraphics[height=1.6cm]{figures/b3-y.png}}; 
        \end{scope}


        


    \end{tikzpicture}
    }
    \end{subfigure}



    \begin{subfigure}[b]{\textwidth}
        \caption{Image-to-Text ICL~\citep{alayrac2022flamingo}}
        \label{fig:demo_micl_text}
    \resizebox{1\textwidth}{!}{%
    \centering
    \begin{tikzpicture}
        \tikzstyle{every node}=[font=\large]
        
        \draw (0,0) pic{myprompt3={MLLM}};
        \node at (1,1) {\includegraphics[height=1.6cm]{figures/chinchilla.png}}; 
        \node at (3,1) {\small\textit{\begin{tabular}{c} This is a \\ chinchilla. They \\ are mainly \\ found in Chile. \end{tabular}}};
        \node at (5,1) {\includegraphics[height=1.6cm]{figures/shiba.png}}; 
        \node at (7,1) {\small\textit{\begin{tabular}{c} This is a shiba. \\ They are very \\ popular in \\ Japan. \end{tabular}}};
        \node at (9,1) {\includegraphics[height=1.6cm]{figures/flamingo.png}}; 
        
        \node at (13.5,1) {\small\textit{\begin{tabular}{c} This is a flamingo. \\ They are found in \\ the Caribbean and \\ South America \end{tabular}}};

    \end{tikzpicture}
    }
    \end{subfigure}
      \end{minipage}
    \hfill
    \begin{minipage}[b]{0.49\linewidth}
    \begin{subfigure}[b]{\textwidth}
    \caption{Text-to-Image ICL~\textbf{(Our Focus)}}
        \label{fig:demo_micl_image}
    \resizebox{1\textwidth}{!}{%
    \centering
    \begin{tikzpicture}
        \tikzstyle{every node}=[font=\large]

        \node at (7.5,3.2) {\LARGE Example Application 1: Interior Decor Design};
        \draw (0,0) pic{myprompt3={MLLM}};

        \node at (1,1) {\begin{tabular}{c}  Study \\ room: \end{tabular}};
        \node at (5,1) {\begin{tabular}{c}  Living \\ room: \end{tabular}};
        \node at (9,1) {\begin{tabular}{c} Bedroom: \end{tabular}};




        \begin{scope}
        \clip (2.2,0.2) rectangle ++(1.6,1.6) ;
        \node at (3,1) {\includegraphics[height=1.6cm]{figures/study_room.jpeg}}; 
        \end{scope}

        \begin{scope}
        \clip (6.2,0.2) rectangle ++(1.6,1.6) ;
        \node at (7,1) {\includegraphics[height=1.6cm]{figures/living_room.jpeg}}; 
        \end{scope}

        \begin{scope}
        \clip (12.7,0.2) rectangle ++(1.6,1.6) ;
        \node at (13.5,1) {\includegraphics[height=1.6cm]{figures/bedroom.png}}; 
        \end{scope}

        \node at (7.5,-0.8) {\LARGE Example Application 2: Product Conceptualization};
        \draw (0,-4) pic{myprompt3={MLLM}};
        \node at (1,-3) {\begin{tabular}{c} Phone: \end{tabular}};
        \node at (5,-3) {\begin{tabular}{c} Tablet: \end{tabular}};
        \node at (9,-3) {\begin{tabular}{c} Car: \end{tabular}};

        \begin{scope}
        \clip (2.2,-3.8) rectangle ++(1.6,1.6) ;
        \node at (3,-3) {\includegraphics[height=1.6cm]{figures/iphone.jpeg}}; 
        \end{scope}

        \begin{scope}
        \clip (6.2,-3.8) rectangle ++(1.6,1.6) ;
        \node at (7,-3) {\includegraphics[height=1.6cm]{figures/ipad.jpeg}}; 
        \end{scope}

        \begin{scope}
        \clip (12.7,-3.8) rectangle ++(1.6,1.6) ;
        \node at (13.5,-3) {\includegraphics[height=1.6cm]{figures/car.png}}; 
        \end{scope}

        \node at (7.5,-4.8) {\LARGE Example Application 3: Anime Character Design};
        \draw (0,-8) pic{myprompt3={MLLM}};
        \node at (1,-7) {\begin{tabular}{c} Optimistic \\ sponge: \end{tabular}};
        \node at (5,-7) {\begin{tabular}{c} Overweight \\ coral-pink \\ starfish: \end{tabular}};
        \node at (9,-7) {\begin{tabular}{c} Arrogrant \\ octopus: \end{tabular}};

        \begin{scope}
        \clip (2.2,-7.8) rectangle ++(1.6,1.6) ;
        \node at (3,-7) {\includegraphics[height=1.6cm]{figures/Spongebob.jpg}}; 
        \end{scope}

        \begin{scope}
        \clip (6.2,-7.8) rectangle ++(1.6,1.6) ;
        \node at (7,-7) {\includegraphics[height=1.6cm]{figures/Patrick.jpg}}; 
        \end{scope}

        \begin{scope}
        \clip (12.7,-7.8) rectangle ++(1.6,1.6) ;
        \node at (13.5,-7) {\includegraphics[height=1.6cm]{figures/squid.png}}; 
        \end{scope}
    \end{tikzpicture}
    }
    \end{subfigure}
     \end{minipage}
    
    \caption{
        \textbf{Comparison of various In-Context Learning (ICL) settings.}
        (a) Textual ICL, where both the input and output in each example are textual. 
        (b) Visual ICL, where both input and output in each demonstration are presented as images.
        (c) Image-to-Text ICL (I2T-ICL), featuring images as input and texts as output in each demonstration.
        (d) Text-to-Image ICL (T2I-ICL, our focus), which involves text input and image output in each demonstration.
        T2I-ICL introduces greater complexities and presents different potential applications.
        The examples in (d) provide three potential applications of T2I-ICL, with the output generated using ChatGPT-4~\citep{openai2023gpt4}, incorporating DALL-E 3~\citep{betker2023dalle3} capabilities.
    }
    \label{fig:intro}
\end{figure*}


==> tex/figures/fig_overview.tex <==
\tikzset{
  pics/myprompt1/.style args={#1,#2,#3,#4}{
     code={
        \path [rounded corners, fill=mycolor1] (2.2,0) rectangle ++(10,2);
        \path [rounded corners, fill=mycolor1] (0,0) rectangle ++(2,2);
        \path [rounded corners, fill=mycolor1] (12.4,0) rectangle ++(2,2);
        \node at (1,1) {\textbf{#1}};
        \node at (3.2,1) {\textbf{#2: }};
        \node at (7.2,1) {\textbf{#3: }};
        \node at (11.2,1) {\textbf{#4: }};

        \begin{scope}
        \clip (4.4,0.2) rectangle ++(1.6,1.6) ;
        \node at (5.2,1) {\includegraphics[height=1.6cm]{tex/datasets/#2_#1}}; 
        \end{scope}
        \begin{scope}
        \clip (8.4,0.2) rectangle ++(1.6,1.6) ;
        \node at (9.2,1) {\includegraphics[height=1.6cm]{tex/datasets/#3_#1}};
        \end{scope}

        \begin{scope}
        \clip (12.6,0.2) rectangle ++(1.6,1.6) ;
        \node at (13.4,1) {\includegraphics[height=1.6cm]{tex/datasets/#4_#1}};
        \end{scope}
     }
  }
}

\tikzset{
  pics/mytask1/.style args={#1,#2,#3,#4,#5,#6,#7,#8,#9}{
     code={
        \draw (0,0) pic{myprompt1={#2,#3,#4,#5}};
        \draw (0,-3) pic{myprompt1={#6,#7,#8,#9}};
        \node [rotate=90] at (1,-0.5) {\textbf{...}};
        \node [rotate=90] at (7.2,-0.5) {\textbf{...}};
        \node [rotate=90] at (13.4,-0.5) {\textbf{...}};
        \path [rounded corners, fill=mycolor2] (-1,-3) rectangle ++(0.8,5);
        \node [rotate=90,text=white] at (-0.6,-0.5) {\textbf{#1}};
        \draw [rounded corners, thick] (-1,-3) rectangle ++(15.4,5);
     }
  }
}

\tikzset{
  pics/myprompt2/.style args={#1,#2,#3,#4}{
     code={
        \path [rounded corners, fill=mycolor1] (2.2,0) rectangle ++(10,2);
        \path [rounded corners, fill=mycolor1] (0,0) rectangle ++(2,2);
        \path [rounded corners, fill=mycolor1] (12.4,0) rectangle ++(2,2);
        \node at (1,1) {\textbf{#1}};
        \node at (3.2,1) {\textbf{#2: }};
        \node at (7.2,1) {\textbf{#3: }};
        \node at (11.2,1) {\textbf{#4: }};

        \begin{scope}
        \clip (4.4,0.2) rectangle ++(1.6,1.6) ;
        \node at (5.2,1) {\includegraphics[height=1.6cm]{tex/datasets/#1_#2}}; 
        \end{scope}
        \begin{scope}
        \clip (8.4,0.2) rectangle ++(1.6,1.6) ;
        \node at (9.2,1) {\includegraphics[height=1.6cm]{tex/datasets/#1_#3}};
        \end{scope}

        \begin{scope}
        \clip (12.6,0.2) rectangle ++(1.6,1.6) ;
        \node at (13.4,1) {\includegraphics[height=1.6cm]{tex/datasets/#1_#4}};
        \end{scope}
     }
  }
}

\tikzset{
  pics/mytask2/.style args={#1,#2,#3,#4,#5,#6,#7,#8,#9}{
     code={
        \draw (0,0) pic{myprompt2={#2,#3,#4,#5}};
        \draw (0,-3) pic{myprompt2={#6,#7,#8,#9}};
        \node [rotate=90] at (1,-0.5) {\textbf{...}};
        \node [rotate=90] at (7.2,-0.5) {\textbf{...}};
        \node [rotate=90] at (13.4,-0.5) {\textbf{...}};
        \path [rounded corners, fill=mycolor2] (-1,-3) rectangle ++(0.8,5);
        \node [rotate=90,text=white] at (-0.6,-0.5) {\textbf{#1}};
        \draw [rounded corners, thick] (-1,-3) rectangle ++(15.4,5);
     }
  }
}

\begin{figure*}[!htb]
    \centering
    \bigskip %
        \resizebox{1\linewidth}{!}{%
    \begin{tikzpicture}
        \tikzstyle{every node}=[font=\large]
        
        \node at (6.7,3.5) {\textbf{\Large Object-Inference Tasks}};
        \path [rounded corners, fill=mycolor2] (0,2.2) rectangle ++(2,0.7);
        \node [text=white] at (1,2.55) {\textbf{Latent Var.}};
        
        \path [rounded corners, fill=mycolor2] (2.2,2.2) rectangle ++(10,0.7);
        \node [text=white] at (7.2,2.55) {\textbf{Prompt}};

        \path [rounded corners, fill=mycolor2] (12.4,2.2) rectangle ++(2,0.7);
        \node [text=white] at (13.4,2.55) {\textbf{Output}};

        \draw (0,0) pic{mytask1={Color-I,Car,White,Blue,Red,Cup,Green,Purple,Orange}};
        \draw (0,-5.2) pic{mytask1={Background-I,Pig,Beach,Desert,Glacier,Zebra,Cave,Space,Waterfall}};
        \draw (0,-10.4) pic{mytask1={Style-I,Apple,Icon,Lego,Origami,Hat,Pixel,Sketch,Graffiti}};
        \draw (0,-15.6) pic{mytask1={Action-I,Cat,Sing,Read,Swim,Dog,Run,Sleep,Fly}};
        \draw (0,-20.8) pic{mytask1={Texture-I,Ball,Metal,Leather,Wood,Box,Wicker,Plastic,Paper}};


        \node at (22.7,3.5) {\Large \textbf{Attribute-Inference Tasks}};
        \path [rounded corners, fill=mycolor2] (16,2.2) rectangle ++(2,0.7);
        \node [text=white] at (17,2.55) {\textbf{Latent Var.}};
        
        \path [rounded corners, fill=mycolor2] (18.2,2.2) rectangle ++(10,0.7);
        \node [text=white] at (23.2,2.55) {\textbf{Prompt}};

        \path [rounded corners, fill=mycolor2] (28.4,2.2) rectangle ++(2,0.7);
        \node [text=white] at (29.4,2.55) {\textbf{Output}};

        \draw (16,0) pic{mytask2={Color-II,Black,Chair,Cup,Box,Pink,Leaf,Car,Book}};
        \draw (16,-5.2) pic{mytask2={Background-II,Volcano,Lion,Zebra,Tiger,Seafloor,Bird,Pig,Monkey}};
        \draw (16,-10.4) pic{mytask2={Style-II,Icon,Hat,Chair,Car,Sketch,Apple,Ball,Leaf}};
        \draw (16,-15.6) pic{mytask2={Action-II,Sleep,Cat,Cow,Lion,Cry,Sheep,Dog,Bird}};
        \draw (16,-20.8) pic{mytask2={Texture-II,Denim,Box,Cup,Apple,Wood,Chair,Ball,Hat}};

        \draw [rounded corners, ultra thick] (-1.2,4) rectangle ++(15.8,-28);
        \draw [rounded corners, ultra thick] (14.8,4) rectangle ++(15.8,-28);
        
    \end{tikzpicture}
    }%

    \caption{
        \textbf{Overview of example prompts in the \ours{} benchmark.} 
        The \ours{} benchmark evaluates the ability of MLLMs to perform T2I-ICL. 
        It covers five themes: color, background, style, action, and texture, each with two different emphases: object-inference and attribute-inference. 
        In object-inference tasks, the attribute (\eg, color) is directly provided in the textual input, and the model is required to infer the object (\eg, car) from the images.
        In other words, the latent variable (denoted as ``Latent Var.'' in the figure) of object-inference tasks is the object.
        Conversely, in attribute-inference tasks, the object is specified in the text.
        The model is tasked with inferring the attribute from the images in the demonstrations, \ie, the attribute serves as the latent variable in attribute-inference tasks. 
        To accomplish the tasks in \ours{}, the models must learn the mapping from the textual input to the corresponding visual output from the demonstrations. 
    }
    \label{fig:overview_data}
\end{figure*}





==> tex/figures/fig_prompt_examples_main_body.tex <==
\tikzset{
  pics/title_img/.style args={#1,#2,#3}{
     code={
        \path [rounded corners, fill=mycolor2] (-2.6,2.1) rectangle ++(2,0.6) node[pos=.5,text=white] {\normalsize Latent Var.};

        \path [rounded corners, fill=mycolor2] (0,2.1) rectangle ++(10.2,0.6) node[pos=.5,text=white] {\normalsize Input};
        
        \path [rounded corners, fill=mycolor2] (10.5,2.1) rectangle ++(2.8,0.6) node[pos=.5,text=white] {\normalsize #1};
        \path [rounded corners, fill=mycolor2] (13.5,2.1) rectangle ++(2.8,0.6) node[pos=.5,text=white] {\normalsize #2};
        \path [rounded corners, fill=mycolor2] (16.5,2.1) rectangle ++(2.8,0.6) node[pos=.5,text=white] {\normalsize #3};
        
     }
  }
}

\tikzset{
  pics/cell_img/.style args={#1,#2}{
     code={
        \draw [rounded corners, fill=mycolor1] (0,0) rectangle ++(2.8,2);

        \begin{scope}
        \clip (0.6,0.2) rectangle ++(1.6,1.6) ;
        \node at (1.4,1) {\includegraphics[height=1.6cm]{#2}}; 
        \end{scope}
        
     }
  }
}

\tikzset{
  pics/row1_img/.style args={#1,#2,#3,#4,#5}{
     code={
        \draw [rounded corners, fill=mycolor1] (-2.6,0) rectangle ++(2,2) node[pos=.5] {\normalsize #1};
        \draw [rounded corners, fill=mycolor1] (0,0) rectangle ++(10.2,2);

        \node at (1,1) {\normalsize #2: };
        \node at (5,1) {\normalsize #3: };
        \node at (9,1) {\normalsize #4: };

        \begin{scope}
        \clip (2.2,0.2) rectangle ++(1.6,1.6) ;
        \node at (3,1) {\includegraphics[height=1.6cm]{tex/datasets/#2_#1.jpg}}; 
        \end{scope}

        \begin{scope}
        \clip (6.2,0.2) rectangle ++(1.6,1.6) ;
        \node at (7,1) {\includegraphics[height=1.6cm]{tex/datasets/#3_#1.jpg}}; 
        \end{scope}
        
        \draw (10.5,0) pic{cell_img={Emu,figures/results/emu_#5_#1_#2_#3_#4.jpg}};
        \draw (13.5,0) pic{cell_img={GILL,figures/results/gill_#5_#1_#2_#3_#4.jpg}};
        \draw (16.5,0) pic{cell_img={SEED-LLaMA,figures/results/seed_#5_#1_#2_#3_#4.jpg}};
        
     }
  }
}

\tikzset{
  pics/row2_img/.style args={#1,#2,#3,#4,#5}{
     code={
        \draw [rounded corners, fill=mycolor1] (-2.6,0) rectangle ++(2,2) node[pos=.5] {\normalsize #1};
        \draw [rounded corners, fill=mycolor1] (0,0) rectangle ++(10.2,2);

        \node at (1,1) {\normalsize #2: };
        \node at (5,1) {\normalsize #3: };
        \node at (9,1) {\normalsize #4: };

        \begin{scope}
        \clip (2.2,0.2) rectangle ++(1.6,1.6) ;
        \node at (3,1) {\includegraphics[height=1.6cm]{tex/datasets/#1_#2.jpg}}; 
        \end{scope}


        \begin{scope}
        \clip (6.2,0.2) rectangle ++(1.6,1.6) ;
        \node at (7,1) {\includegraphics[height=1.6cm]{tex/datasets/#1_#3.jpg}}; 
        \end{scope}
        
        \draw (10.5,0) pic{cell_img={Emu,figures/results/emu_#5_#1_#2_#3_#4.jpg}};
        \draw (13.5,0) pic{cell_img={GILL,figures/results/gill_#5_#1_#2_#3_#4.jpg}};       
        \draw (16.5,0) pic{cell_img={SEED-LLaMA,figures/results/seed_#5_#1_#2_#3_#4.jpg}};
        
     }
  }
}

\tikzset{
  pics/cell_text/.style args={#1,#2}{
     code={
        \draw [rounded corners, fill=mycolor1] (0,0) rectangle ++(6,3);
        \node[text width=5cm] at (3,1.4) {\textit{\normalsize #2}};
        \path [rounded corners, fill=mycolor2] (0,3.1) rectangle ++(6,0.6) node[pos=.5,text=white] {\normalsize #1};
        
     }
  }
}

\tikzset{
  pics/row1_text/.style args={#1,#2,#3,#4}{
     code={
        \path [rounded corners, fill=mycolor2] (0,2.1) rectangle ++(2,0.6) node[pos=.5,text=white] {\normalsize Latent Var.};
        \path [rounded corners, fill=mycolor2] (2.2,2.1) rectangle ++(10,0.6) node[pos=.5,text=white] {\normalsize Input};

        \draw [rounded corners, fill=mycolor1] (0,0) rectangle ++(2,2) node[pos=.5] {\normalsize #1};
        \draw [rounded corners, fill=mycolor1] (2.2,0) rectangle ++(10,2);

        \node at (3.2,1) {\normalsize #2: };
        \node at (7.2,1) {\normalsize #3: };
        \node at (11.2,1) {\normalsize #4: };

        \begin{scope}
        \clip (4.4,0.2) rectangle ++(1.6,1.6) ;
        \node at (5.2,1) {\includegraphics[height=1.6cm]{tex/datasets/#2_#1.jpg}}; 
        \end{scope}

        \begin{scope}
        \clip (8.4,0.2) rectangle ++(1.6,1.6) ;
        \node at (9.2,1) {\includegraphics[height=1.6cm]{tex/datasets/#3_#1.jpg}}; 
        \end{scope}        
     }
  }
}

\tikzset{
  pics/row2_text/.style args={#1,#2,#3,#4}{
     code={
        \path [rounded corners, fill=mycolor2] (0,2.1) rectangle ++(2,0.6) node[pos=.5,text=white] {\normalsize Latent Var.};
        \path [rounded corners, fill=mycolor2] (2.2,2.1) rectangle ++(10,0.6) node[pos=.5,text=white] {\normalsize Input};

        \draw [rounded corners, fill=mycolor1] (0,0) rectangle ++(2,2) node[pos=.5] {\normalsize #1};
        \draw [rounded corners, fill=mycolor1] (2.2,0) rectangle ++(10,2);

        \node at (3.2,1) {\normalsize #2: };
        \node at (7.2,1) {\normalsize #3: };
        \node at (11.2,1) {\normalsize #4: };

        \begin{scope}
        \clip (4.4,0.2) rectangle ++(1.6,1.6) ;
        \node at (5.2,1) {\includegraphics[height=1.6cm]{tex/datasets/#1_#2.jpg}}; 
        \end{scope}

        \begin{scope}
        \clip (8.4,0.2) rectangle ++(1.6,1.6) ;
        \node at (9.2,1) {\includegraphics[height=1.6cm]{tex/datasets/#1_#3.jpg}}; 
        \end{scope}
     }
  }
}

\begin{figure*}[!htb]

    \begin{subfigure}[b]{\linewidth}
        \centering
        \resizebox{\linewidth}{!}{%
            \begin{tikzpicture}
            \tikzstyle{every node}=[font=\large]
    
            \draw (0,0) pic{title_img={Emu,GILL,SEED-LLaMA}};
    
            \draw (0,0) pic{row1_img={Bag,Brown,Blue,Purple,873}};
            \draw (0,-2.1) pic{row1_img={Car,Brown,Purple,Orange,519}};
            \draw (0,-4.2) pic{row1_img={Hat,Green,Yellow,White,893}};
            \draw (0,-6.3) pic{row1_img={Book,Purple,White,Pink,324}};
            \draw (0,-8.4) pic{row1_img={Box,White,Yellow,Green,655}};
            \draw (0,-10.5) pic{row1_img={Leaf,Pink,Brown,Blue,445}};
    
        \end{tikzpicture}
        }
        \caption{Image generation.}
    \end{subfigure}
    \begin{subfigure}[b]{\linewidth}
        \centering
        \resizebox{\linewidth}{!}{%
            \begin{tikzpicture}
            \tikzstyle{every node}=[font=\large]
    
            \draw (0,0.3) pic{row1_text={Bag,Brown,Blue,Purple}}; %
            
            \draw (0,-4) pic{cell_text={Emu,A brown leather backpack with two zippers.}};
            \draw (6.2,-4) pic{cell_text={GILL,image of the backpack in the image
            }};
            \draw (0,-8) pic{cell_text={SEED-LLaMA,I have generated an image.}};
            \draw (6.2,-8) pic{cell_text={LLaVA,The next image should be a close-up of a blue backpack with a brown strap.}};
            \draw (0,-12) pic{cell_text={Qwen-VL,The next image should be a close-up of a blue backpack with brown leather details, showcasing the main object clearly.}};
            \draw (6.2,-12) pic{cell_text={GPT-4V,A purple backpack with a similar style to the previous images, featuring a vibrant purple fabric, sturdy zippers}};


            \draw [] (12.6,3) to (12.6,-12);

            \draw (13,0.3) pic{row1_text={Car,Brown,Purple,Orange}}; %
            
            \draw (13,-4) pic{cell_text={Emu,An orange sports car driving down a road.}};
            \draw (19.2,-4) pic{cell_text={GILL,automobile model is a car that is a sports car}};
            \draw (13,-8) pic{cell_text={SEED-LLaMA,I have generated an image.}};
            \draw (19.2,-8) pic{cell_text={LLaVA,The next image should be a close-up of the front of the purple sports car, showcasing its grill and headlights. The car should be parked on a street,  }};
            \draw (13,-12) pic{cell_text={Qwen-VL,The next image should be an orange sports car driving on a road with a blurry background.}};
            \draw (19.2,-12) pic{cell_text={GPT-4V,A sleek race car in bright orange, with black detailing, glossy finish, and racing stripes, speeding on a racetrack with motion blur in the background.}};
        \end{tikzpicture}
        }
        \caption{Image description generation.}
    \end{subfigure}
    \caption{Examples of prompts and corresponding images and image descriptions generated by MLLMs for task Color-I.}
    \label{fig:example_prompt_results_main}
\end{figure*}


